Maximum weighted induced forests and trees: New formulations and a computational comparative review

Given a graph $G=(V,E)$ with a weight $w_v$ associated with each vertex $v\in V$, the maximum weighted induced forest problem (MWIF) consists of encountering a maximum weighted subset $V'\subseteq V$ of the vertices such that $V'$ induces a forest. This NP-hard problem is known to be equivalent to the minimum weighted feedback vertex set problem, which has applicability in a variety of domains. The closely related maximum weighted induced tree problem (MWIT), on the other hand, requires that the subset $V'\subseteq V$ induces a tree. We propose two new integer programming formulations with an exponential number of constraints and branch-and-cut procedures for MWIF. Computational experiments using benchmark instances are performed comparing several formulations, including the newly proposed approaches and those available in the literature, when solved by a standard commercial mixed integer programming solver. More specifically, five formulations are compared, two compact (i.e., with a polynomial number of variables and constraints) ones and the three others with an exponential number of constraints. The experiments show that a new formulation for the problem based on directed cutset inequalities for eliminating cycles (DCUT) offers stronger linear relaxation bounds earlier in the search process. The results also indicate that the other new formulation, denoted tree with cycle elimination (TCYC), outperforms those available in the literature when it comes to the average times for proving optimality for the small instances, especially the more challenging ones. Additionally, this formulation can achieve much lower average times for solving the larger random instances that can be optimally solved. Furthermore, we show how the formulations for MWIF can be easily extended for MWIT. Such extension allowed us to compare the optimal solution values of the two problems.

==> 99_old_computationalresults.tex <==
\section{Computational experiments}
\label{sec:experiments}

In this section, we summarize the computational experiments performed to assess the effectiveness
%\celsoF{A verificar: efficiency?}\rafaelF{Quando falo de algoritmos ou formulações, evito falar de efficient por questões de ambiguidade com conceitos de eficiência de algoritmos. Se achar que não tem problema, podemos mudar.}\celsoF{E a que você se refere aqui? Estamos comparando eficiência (tempo) ou eficácia (capacidade de encontrar boas soluções)?}\rafaelF{Na verdade, um pouco dos dois. Primeiro instâncias resolvidas, depois tempo. O meu medo maior de ambiguidade é menos relacionado a questão de tempo, mas sim a complexidade.} 
of the formulations described in Section~\ref{sec:formulations}.
All computational experiments were carried out on a machine running under Ubuntu GNU/Linux, with an Intel(R) Core(TM) i7-4770 CPU @ 3.40GHz processor and 16Gb of RAM. The algorithms were coded in Julia v1.4.2, using JuMP v0.18.6. The formulations were solved using Gurobi 9.0.2.

\subsection{Instances}
\label{sec:instancias}

The experiments were performed using the benchmark instances proposed in \citeA{CarCerGen11} for the maximum weighted feedback vertex set problem, where more details can be encountered. The instances are available in~\citeA{instances}. They consist of random, grid, toroidal, and hypercube graphs, and are classified as small, with $16 \leq |V| \leq 81$, or large,  with $91 \leq |V| \leq 529$. The node weights are uniformly distributed in one of the following intervals: $[10,25]$, $[10,50]$, or $[10,75]$. Similar instances, but with different weights, are organized into instance groups containing five instances each. Each instance group is identified as $X\_n\_m\_low\_up$, where $X$ gives the class of the graph: square grid ($G$), non-square grid ($\mathit{GNQ}$), hypercube ($H$), toroidal ($T$), or random ($R$). 
For random graphs $n$ and $m$ denote, respectively, the numbers of vertices and edges;
for grid and toroidal graphs $n$ and $m$ denote, correspondingly, the number of lines and columns of the grid; 
for hypercube graphs $n=m$ identifies the corresponding $n$-hypercube graph;
the other parameters indicate the lower ($\mathit{low}$) and upper ($\mathit{up}$) bounds on the weights.  
We remark that the results reported throughout this section represent average values over the five instances belonging to the same instance group. 

\subsection{Tested approaches and settings}
\label{sec:testedapproaches}

The following approaches were considered in our experiments:
\begin{itemize}
    \item cycle elimination formulation (CYC) strengthened with clique inequalities; 
    \item tree with cycle elimination formulation (TCYC) strengthened with clique inequalities;
    \item compact flow-based formulation (FLOW);
    \item compact MTZ-based formulation (MTZ); and
    \item directed cutset formulation (DCUT) strengthened with clique inequalities.
\end{itemize}

\rafaelC{Note that we follow a common practice in the literature. Namely, FLOW and MTZ are only tested as plain formulations, i.e., without our branch-and-cut procedures. The reason for that is to keep the formulations compact. This makes them a viable option for being easily implemented by a practitioner as one does not have to resort to more advanced algorithmic implementations.}

The MIP solver was executed using the standard configurations, except the relative optimality tolerance gap which was set to $10^{-6}$. A time limit of 3600 seconds was imposed for each execution of the MIP solver. All the separation procedures were implemented as callbacks in the MIP solver. \rafaelC{To avoid overloading the formulation with an excessive amount of cuts throughout the search tree, the} separations for fractional solutions were only executed at the root node. Each formulation was tested (a)\rafaelF{Que tal removermos o (a) e deixarmos somente o resultado com a solução inicial??} as a standalone approach and (b) receiving as input a good quality warm start (i.e., a feasible solution) generated by the matheuristic MILS$^+$-$mtz$ described in Section 3.6 of~\citeA{MelQueRib21}.

We remark that \citeA{BruMafTru00} also showed that certain subset inequalities are valid for the feedback vertex set problem. However, the authors observed in the computational experiments that these inequalities slowed down the solution process and, for this reason, we did not use such inequalities in our experiments.

\subsection{Small instances}
\label{sec:smallinstances}

Tables~\ref{tab:grid}-\ref{tab:randominitsol} summarize the results for the small instances, with Tables~\ref{tab:grid}-\ref{tab:rand} corresponding to the formulations as standalone approaches and Tables~\ref{tab:gridinitsol}-\ref{tab:randominitsol} to the formulations when offered warm starts.
In each of these tables, the first column identifies the instance group. Next, for each of the approaches (CYC, TCYC, FLOW, MTZ, and DCUT), the tables show the average best value (avg), the number of instances solved to optimality (opt) followed by the average time to solve them (time), and the average relative open gap (gap) in percent considering the instances which were not solved to optimality, given by $100\times \frac{ub-lb}{ub}$, where $ub$ gives the best bound and $lb$ the best solution value.
Whenever the majority (i.e., at least three) of the formulations are able to solve the same amount of instances, the best average time \rafaelC{is shown in bold}. Otherwise, the maximum number of instances solved to optimality appears \rafaelC{in bold} and, in case no instances were solved to optimality by any of the formulations, the smallest gap is represented \rafaelC{in bold}.


%\celsoF{Mas já vou deixar um comentário sobre o que me parece estar faltando: figuras e gráficos. Ajudaram muito no artigo com Michell. Vamos pensar nisso a medida em que eu avanço na revisão, se podemos fazer uns gráficos de barras como os que ele fez pelas categorias e por ALL de instâncias. Ou ainda umas figuras ilustrativas simples com grafos no início do artigo, como as Figuras 1 a 3 do artigo com Michell. Acho que deixa mais leve. Eu me lembro que a Lilian sempre dizia que artigo sobre grafos tem que ter grafo desenhado.}

Tables~\ref{tab:grid}~and~\ref{tab:gridnq} show that all small grid instances could be solved to optimality using all the five formulations, most of them in low computational times. It can be noted that FLOW achieved the lowest average times for most of the instance groups, while DCUT needed more time on average to solve these instances.
Table~\ref{tab:ipercube} shows that, for the small hypercube instances, all formulations but CYC were able to solve all instances to optimality. TCYC achieved the lower average times. 
%and 
It can also be noted that the average times for FLOW and MTZ are very similar for these instances.
Table~\ref{tab:toro} shows that, for the small toroidal instances, all formulations but CYC solved all instances to optimality, with FLOW achieving lower average times.
Table~\ref{tab:rand} shows that for the small random instances, again, all formulations but CYC were able to solve all of them to optimality, with TCYC achieving lower average times, followed by DCUT. It can be seen that, for these instances, TCYC and DCUT outperformed by far MTZ and FLOW, especially for the larger instances in the subset, indicating the benefits of a branch-and-cut approach using the formulations with clique inequalities.

%SAIU DAQUI

\begin{landscape}


% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Fri Aug 28 18:19:35 2020
\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations for the small square grid instances.}\label{tab:grid}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
G\_5\_5\_10\_25 & 352.4 & 5 & 1.4 &  & 352.4 & 5 & 1.1 &  & 352.4 & 5 & \textbf{0.1} &  & 352.4 & 5 & \textbf{0.1} &  & 352.4 & 5 & 1.7 &  \\ 
  G\_5\_5\_10\_50 & 636.8 & 5 & 1.4 &  & 636.8 & 5 & 1.1 &  & 636.8 & 5 & \textbf{0.1} &  & 636.8 & 5 & \textbf{0.1} &  & 636.8 & 5 & 1.8 &  \\ 
  G\_5\_5\_10\_75 & 934.2 & 5 & 1.4 &  & 934.2 & 5 & 1.1 &  & 934.2 & 5 & \textbf{0.1} &  & 934.2 & 5 & \textbf{0.1} &  & 934.2 & 5 & 1.8 &  \\ \hline
  G\_7\_7\_10\_25 & 712.4 & 5 & 1.5 &  & 712.4 & 5 & 1.2 &  & 712.4 & 5 & \textbf{0.3} &  & 712.4 & 5 & 0.7 &  & 712.4 & 5 & 2.4 &  \\ 
  G\_7\_7\_10\_50 & 1324.2 & 5 & 1.5 &  & 1324.2 & 5 & 1.1 &  & 1324.2 & 5 & \textbf{0.3} &  & 1324.2 & 5 & \textbf{0.3} &  & 1324.2 & 5 & 2.1 &  \\ 
  G\_7\_7\_10\_75 & 1998.6 & 5 & 1.5 &  & 1998.6 & 5 & 1.2 &  & 1998.6 & 5 & \textbf{0.3} &  & 1998.6 & 5 & 0.4 &  & 1998.6 & 5 & 2.1 &  \\ \hline
  G\_9\_9\_10\_25 & 1180.8 & 5 & 6.3 &  & 1180.8 & 5 & \textbf{1.8} &  & 1180.8 & 5 & 2.3 &  & 1180.8 & 5 & 10.1 &  & 1180.8 & 5 & 177.3 &  \\ 
  G\_9\_9\_10\_50 & 2192.2 & 5 & 2.5 &  & 2192.2 & 5 & \textbf{1.3} &  & 2192.2 & 5 & 1.4 &  & 2192.2 & 5 & 2.8 &  & 2192.2 & 5 & 249.5 &  \\ 
  G\_9\_9\_10\_75 & 3452.2 & 5 & 2.4 &  & 3452.2 & 5 & 1.3 &  & 3452.2 & 5 & \textbf{1.1} &  & 3452.2 & 5 & 1.4 &  & 3452.2 & 5 & 86.7 &  \\ \hline
  Average & 1420.4 &  & 2.2 &  & 1420.4 &  & 1.2 &  & 1420.4 &  & 0.7 &  & 1420.4 &  & 1.8 &  & 1420.4 &  & 58.4 &  \\ 
  Total &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  \\ 
   \hline
\end{tabular}
\end{table}




% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Fri Aug 28 18:24:57 2020
\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations for the small non-square grid instances.}\label{tab:gridnq}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
GNQ\_8\_3\_10\_25 & 319.2 & 5 & 1.4 &  & 319.2 & 5 & 1.1 &  & 319.2 & 5 & \textbf{0.1} &  & 319.2 & 5 & \textbf{0.1} &  & 319.2 & 5 & 1.8 &  \\ 
  GNQ\_8\_3\_10\_50 & 579.2 & 5 & 1.4 &  & 579.2 & 5 & 1.1 &  & 579.2 & 5 & \textbf{0.0} &  & 579.2 & 5 & 0.1 &  & 579.2 & 5 & 1.8 &  \\ 
  GNQ\_8\_3\_10\_75 & 838.0 & 5 & 1.3 &  & 838.0 & 5 & 1.1 &  & 838.0 & 5 & \textbf{0.0} &  & 838.0 & 5 & 0.1 &  & 838.0 & 5 & 1.8 &  \\ \hline
  GNQ\_9\_6\_10\_25 & 786.8 & 5 & 1.7 &  & 786.8 & 5 & 1.2 &  & 786.8 & 5 & \textbf{0.4} &  & 786.8 & 5 & 2.3 &  & 786.8 & 5 & 2.3 &  \\ 
  GNQ\_9\_6\_10\_50 & 1438.6 & 5 & 1.5 &  & 1438.6 & 5 & 1.2 &  & 1438.6 & 5 & \textbf{0.4} &  & 1438.6 & 5 & 0.7 &  & 1438.6 & 5 & 16.2 &  \\ 
  GNQ\_9\_6\_10\_75 & 2195.6 & 5 & 1.5 &  & 2195.6 & 5 & 1.2 &  & 2195.6 & 5 & \textbf{0.4} &  & 2195.6 & 5 & 0.6 &  & 2195.6 & 5 & 4.5 &  \\ \hline
  GNQ\_12\_6\_10\_25 & 1071.2 & 5 & 2.8 &  & 1071.2 & 5 & 1.3 &  & 1071.2 & 5 & \textbf{1.2} &  & 1071.2 & 5 & 5.0 &  & 1071.2 & 5 & 38.0 &  \\ 
  GNQ\_12\_6\_10\_50 & 1944.2 & 5 & 1.9 &  & 1944.2 & 5 & 1.3 &  & 1944.2 & 5 & \textbf{1.1} &  & 1944.2 & 5 & 2.8 &  & 1944.2 & 5 & 250.9 &  \\ 
  GNQ\_12\_6\_10\_75 & 3022.4 & 5 & 1.7 &  & 3022.4 & 5 & 1.2 &  & 3022.4 & 5 & \textbf{0.8} &  & 3022.4 & 5 & 1.8 &  & 3022.4 & 5 & 32.8 &  \\ 
   \hline
      Average & 1355.0 &  & 1.7 &  & 1355.0 &  & 1.2 &  & 1355.0 &  & 0.5 &  & 1355.0 &  & 1.5 &  & 1355.0 &  & 38.9 &  \\ 
  Total &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  \\ 
   \hline
\end{tabular}
\end{table}





% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Fri Aug 28 17:46:35 2020
\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations for the small hypercube instances.}\label{tab:ipercube}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
I\_4\_10\_25 & 147.0 & 5 & 1.4 &  & 147.0 & 5 & 1.1 &  & 147.0 & 5 & \textbf{0.0} &  & 147.0 & 5 & 0.1 &  & 147.0 & 5 & 1.8 &  \\ 
  I\_4\_10\_50 & 289.4 & 5 & 1.4 &  & 289.4 & 5 & 1.1 &  & 289.4 & 5 & \textbf{0.0} &  & 289.4 & 5 & \textbf{0.0} &  & 289.4 & 5 & 1.8 &  \\ 
  I\_4\_10\_75 & 344.0 & 5 & 1.4 &  & 344.0 & 5 & 1.1 &  & 344.0 & 5 & \textbf{0.0} &  & 344.0 & 5 & \textbf{0.0} &  & 344.0 & 5 & 1.7 &  \\ \hline
  I\_5\_10\_25 & 278.4 & 5 & 2.3 &  & 278.4 & 5 & 1.3 &  & 278.4 & 5 & 0.8 &  & 278.4 & 5 & \textbf{0.7} &  & 278.4 & 5 & 2.8 &  \\ 
  I\_5\_10\_50 & 545.0 & 5 & 1.5 &  & 545.0 & 5 & 1.2 &  & 545.0 & 5 & \textbf{0.2} &  & 545.0 & 5 & \textbf{0.2} &  & 545.0 & 5 & 1.9 &  \\ 
  I\_5\_10\_75 & 787.4 & 5 & 1.5 &  & 787.4 & 5 & 1.1 &  & 787.4 & 5 & \textbf{0.1} &  & 787.4 & 5 & \textbf{0.1} &  & 787.4 & 5 & 1.9 &  \\ \hline
  I\_6\_10\_25 & 527.2 & 3 & 2871.4 & 3.1 & 527.2 & 5 & \textbf{23.9} &  & 527.2 & 5 & 66.3 &  & 527.2 & 5 & 67.1 &  & 527.2 & 5 & 1767.4 &  \\ 
  I\_6\_10\_50 & 975.6 & 5 & 22.5 &  & 975.6 & 5 & \textbf{2.8} &  & 975.6 & 5 & 5.2 &  & 975.6 & 5 & 4.2 &  & 975.6 & 5 & 152.0 &  \\ 
  I\_6\_10\_75 & 1250.8 & 5 & 7.1 &  & 1250.8 & 5 & 1.4 &  & 1250.8 & 5 & 1.0 &  & 1250.8 & 5 & \textbf{0.7} &  & 1250.8 & 5 & 3.2 &  \\ 
   \hline
  Average & 571.6 &  & 323.4 & 3.1 & 571.6 &  & 3.9 &  & 571.6 &  & 8.2 &  & 571.6 &  & 8.1 &  & 571.6 &  & 215.0 &  \\ 
  Total &  & 43 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  \\ 
   \hline
\end{tabular}
\end{table}



% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Fri Aug 28 17:58:35 2020
\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations for the small toroidal instances.}\label{tab:toro}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
T\_5\_5\_10\_25 & 232.8 & 5 & 1.5 &  & 232.8 & 5 & 1.1 &  & 232.8 & 5 & \textbf{0.1} &  & 232.8 & 5 & \textbf{0.1} &  & 232.8 & 5 & 1.8 &  \\ 
  T\_5\_5\_10\_50 & 357.2 & 5 & 1.4 &  & 357.2 & 5 & 1.2 &  & 357.2 & 5 & \textbf{0.1} &  & 357.2 & 5 & \textbf{0.1} &  & 357.2 & 5 & 1.8 &  \\ 
  T\_5\_5\_10\_75 & 448.6 & 5 & 1.4 &  & 448.6 & 5 & 1.1 &  & 448.6 & 5 & \textbf{0.1} &  & 448.6 & 5 & \textbf{0.1} &  & 448.6 & 5 & 1.8 &  \\ \hline
  T\_7\_7\_10\_25 & 471.2 & 5 & 4.9 &  & 471.2 & 5 & 1.3 &  & 471.2 & 5 & \textbf{0.6} &  & 471.2 & 5 & 0.8 &  & 471.2 & 5 & 2.5 &  \\ 
  T\_7\_7\_10\_50 & 734.6 & 5 & 1.7 &  & 734.6 & 5 & 1.2 &  & 734.6 & 5 & \textbf{0.3} &  & 734.6 & 5 & 0.4 &  & 734.6 & 5 & 2.2 &  \\ 
  T\_7\_7\_10\_75 & 912.4 & 5 & 1.7 &  & 912.4 & 5 & 1.2 &  & 912.4 & 5 & 0.4 &  & 912.4 & 5 & \textbf{0.3} &  & 912.4 & 5 & 2.3 &  \\ \hline
  T\_9\_9\_10\_25 & 730.0 & 0 &  & 2.0 & 730.0 & 5 & 10.5 &  & 730.0 & 5 & \textbf{5.4} &  & 730.0 & 5 & 12.6 &  & 730.0 & 5 & 50.0 &  \\ 
  T\_9\_9\_10\_50 & 1130.4 & 5 & 50.5 &  & 1130.4 & 5 & 1.9 &  & 1130.4 & 5 & \textbf{1.2} &  & 1130.4 & 5 & 2.9 &  & 1130.4 & 5 & 132.2 &  \\ 
  T\_9\_9\_10\_75 & 1478.6 & 5 & 16.2 &  & 1478.6 & 5 & 1.7 &  & 1478.6 & 5 & \textbf{1.1} &  & 1478.6 & 5 & 1.2 &  & 1478.6 & 5 & 49.0 &  \\ 
   \hline
 Average & 721.8 &  & 9.9 & 2.0 & 721.8 &  & 2.4 &  & 721.8 &  & 1.0 &  & 721.8 &  & 2.1 &  & 721.8 &  & 27.1 &  \\ 
  Total &  & 40 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  \\ 
   \hline
\end{tabular}
\end{table}


% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Fri Aug 28 15:15:12 2020
\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations for the small random instances.}\label{tab:rand}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
R\_25\_33\_10\_25 & 317.2 & 5 & 1.4 &  & 317.2 & 5 & 1.1 &  & 317.2 & 5 & \textbf{0.0} &  & 317.2 & 5 & 0.1 &  & 317.2 & 5 & 1.8 &  \\ 
  R\_25\_33\_10\_50 & 525.8 & 5 & 1.4 &  & 525.8 & 5 & 1.1 &  & 525.8 & 5 & \textbf{0.0} &  & 525.8 & 5 & 0.1 &  & 525.8 & 5 & 1.8 &  \\ 
  R\_25\_33\_10\_75 & 702.8 & 5 & 1.4 &  & 702.8 & 5 & 1.1 &  & 702.8 & 5 & \textbf{0.0} &  & 702.8 & 5 & 0.1 &  & 702.8 & 5 & 1.4 &  \\ \hline 
  R\_25\_69\_10\_25 & 243.0 & 5 & 1.5 &  & 243.0 & 5 & 1.2 &  & 243.0 & 5 & 0.2 &  & 243.0 & 5 & \textbf{0.1} &  & 243.0 & 5 & 1.9 &  \\ 
  R\_25\_69\_10\_50 & 389.8 & 5 & 1.5 &  & 389.8 & 5 & 1.2 &  & 389.8 & 5 & \textbf{0.2} &  & 389.8 & 5 & \textbf{0.2} &  & 389.8 & 5 & 1.9 &  \\ 
  R\_25\_69\_10\_75 & 597.2 & 5 & 1.5 &  & 597.2 & 5 & 1.2 &  & 597.2 & 5 & 0.2 &  & 597.2 & 5 & \textbf{0.1} &  & 597.2 & 5 & 1.9 &  \\ \hline 
  R\_25\_204\_10\_25 & 106.8 & 5 & 1.8 &  & 106.8 & 5 & 1.6 &  & 106.8 & 5 & 1.7 &  & 106.8 & 5 & \textbf{1.0} &  & 106.8 & 5 & 2.2 &  \\ 
  R\_25\_204\_10\_50 & 193.0 & 5 & 1.7 &  & 193.0 & 5 & 1.5 &  & 193.0 & 5 & 1.3 &  & 193.0 & 5 & \textbf{0.8} &  & 193.0 & 5 & 2.2 &  \\ 
  R\_25\_204\_10\_75 & 312.2 & 5 & 1.7 &  & 312.2 & 5 & 1.5 &  & 312.2 & 5 & 1.4 &  & 312.2 & 5 & \textbf{0.7} &  & 312.2 & 5 & 2.2 &  \\ \hline 
  R\_50\_85\_10\_25 & 583.2 & 5 & 2.7 &  & 583.2 & 5 & 1.2 &  & 583.2 & 5 & \textbf{0.2} &  & 583.2 & 5 & 0.3 &  & 583.2 & 5 & 2.1 &  \\ 
  R\_50\_85\_10\_50 & 957.2 & 5 & 1.9 &  & 957.2 & 5 & 1.2 &  & 957.2 & 5 & \textbf{0.2} &  & 957.2 & 5 & 0.4 &  & 957.2 & 5 & 2.0 &  \\ 
  R\_50\_85\_10\_75 & 1229.8 & 5 & 1.7 &  & 1229.8 & 5 & 1.2 &  & 1229.8 & 5 & \textbf{0.2} &  & 1229.8 & 5 & 0.3 &  & 1229.8 & 5 & 2.0 &  \\ \hline 
  R\_50\_232\_10\_25 & 355.2 & 5 & 92.8 &  & 355.2 & 5 & \textbf{2.1} &  & 355.2 & 5 & 5.7 &  & 355.2 & 5 & 3.4 &  & 355.2 & 5 & 4.9 &  \\ 
  R\_50\_232\_10\_50 & 657.2 & 5 & 38.6 &  & 657.2 & 5 & \textbf{1.8} &  & 657.2 & 5 & 4.9 &  & 657.2 & 5 & 3.1 &  & 657.2 & 5 & 4.3 &  \\ 
  R\_50\_232\_10\_75 & 889.6 & 5 & 35.4 &  & 889.6 & 5 & \textbf{1.8} &  & 889.6 & 5 & 4.6 &  & 889.6 & 5 & 2.6 &  & 889.6 & 5 & 4.3 &  \\ \hline 
  R\_50\_784\_10\_25 & 146.4 & 5 & 189.5 &  & 146.4 & 5 & 15.0 &  & 146.4 & 5 & 39.3 &  & 146.4 & 5 & 42.7 &  & 146.4 & 5 & \textbf{12.7} &  \\ 
  R\_50\_784\_10\_50 & 278.2 & 5 & 147.0 &  & 278.2 & 5 & 15.9 &  & 278.2 & 5 & 33.3 &  & 278.2 & 5 & 40.8 &  & 278.2 & 5 & \textbf{11.9} &  \\ 
  R\_50\_784\_10\_75 & 415.6 & 5 & 110.3 &  & 415.6 & 5 & 11.3 &  & 415.6 & 5 & 32.9 &  & 415.6 & 5 & 32.1 &  & 415.6 & 5 & \textbf{9.0} &  \\ \hline 
  R\_75\_157\_10\_25 & 792.0 & 5 & 861.1 &  & 792.0 & 5 & 3.6 &  & 792.0 & 5 & \textbf{1.2} &  & 792.0 & 5 & 3.0 &  & 792.0 & 5 & 6.1 &  \\ 
  R\_75\_157\_10\_50 & 1250.6 & 5 & 312.7 &  & 1250.6 & 5 & 2.9 &  & 1250.6 & 5 & \textbf{1.2} &  & 1250.6 & 5 & 1.3 &  & 1250.6 & 5 & 4.2 &  \\ 
  R\_75\_157\_10\_75 & 1870.6 & 5 & 84.4 &  & 1870.6 & 5 & 1.8 &  & 1870.6 & 5 & \textbf{1.1} &  & 1870.6 & 5 & \textbf{1.1} &  & 1870.6 & 5 & 15.2 &  \\ \hline 
  R\_75\_490\_10\_25 & 460.2 & 0 &  & 13.9 & 461.8 & 5 & \textbf{31.1} &  & 461.8 & 5 & 163.9 &  & 461.8 & 5 & 137.2 &  & 461.8 & 5 & 74.9 &  \\ 
  R\_75\_490\_10\_50 & 776.4 & 0 &  & 18.5 & 797.4 & 5 & \textbf{24.6} &  & 797.4 & 5 & 219.9 &  & 797.4 & 5 & 117.8 &  & 797.4 & 5 & 82.8 &  \\ 
  R\_75\_490\_10\_75 & 1212.2 & 0 &  & 12.8 & 1233.4 & 5 & \textbf{12.6} &  & 1233.4 & 5 & 115.7 &  & 1233.4 & 5 & 53.4 &  & 1233.4 & 5 & 38.1 &  \\ \hline 
  R\_75\_1739\_10\_25 & 154.4 & 0 &  & 43.5 & 158.4 & 5 & \textbf{159.8} &  & 158.4 & 5 & 827.8 &  & 158.4 & 5 & 464.6 &  & 158.4 & 5 & 185.3 &  \\ 
  R\_75\_1739\_10\_50 & 295.6 & 0 &  & 38.9 & 300.4 & 5 & 120.1 &  & 300.4 & 5 & 708.6 &  & 300.4 & 5 & 339.9 &  & 300.4 & 5 & \textbf{112.7} &  \\ 
  R\_75\_1739\_10\_75 & 454.2 & 0 &  & 31.0 & 458.2 & 5 & 117.1 &  & 458.2 & 5 & 658.2 &  & 458.2 & 5 & 321.7 &  & 458.2 & 5 & \textbf{114.7} &  \\ 
   \hline
     Average & 598.8 &  & 90.1 & 26.4 & 600.9 &  & 19.9 &  & 600.9 &  & 104.6 &  & 600.9 &  & 58.1 &  & 600.9 &  & 26.1 &  \\ 
  Total &  & 105 &  &  &  & 135 &  &  &  & 135 &  &  &  & 135 &  &  &  & 135 &  &  \\ 
   \hline
\end{tabular}
\end{table}


\end{landscape}


Tables~\ref{tab:gridinitsol}-\ref{tab:randominitsol} summarize the results for the small instances when receiving a warm start. Tables~\ref{tab:gridinitsol}~and~\ref{tab:gridnqinitsol} show that all approaches but DCUT presented similar results to those without a warm start for the small grid instances. DCUT achieved large reductions in average times, what indicates that when using such formulation without a warm start, the solver encountered difficulties in finding good quality feasible solutions.
Table~\ref{tab:ipercubeinitsol} shows that, for the hypercube instances, offering a warm start did not allow significant improvements using any of the formulations. On the contrary, one less instance was solved to optimality with CYC.
Table~\ref{tab:toroinitsol} shows that, similarly to the grid instances, offering a warm start to DCUT allowed significant reductions on the average times to solve small toroidal instances to optimality.
Table~\ref{tab:randominitsol} shows that, for the small random instances, reasonable reductions were achieved when providing a warm start for all approaches when it comes to the average times, with TCYC and DCUT remaining as the best approaches for this subset of instances. Besides, the warm start enhanced the advantage of TCYC over the other approaches for these instances.


\begin{landscape}


\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations with warm start for the small square grid instances.}\label{tab:gridinitsol}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
G\_5\_5\_10\_25 & 352.4 & 5 & 1.4 &  & 352.4 & 5 & 1.1 &  & 352.4 & 5 & \textbf{0.1} &  & 352.4 & 5 & \textbf{0.1} &  & 352.4 & 5 & 1.6 &  \\ 
  G\_5\_5\_10\_50 & 636.8 & 5 & 1.4 &  & 636.8 & 5 & 1.1 &  & 636.8 & 5 & \textbf{0.1} &  & 636.8 & 5 & \textbf{0.1} &  & 636.8 & 5 & 1.6 &  \\ 
  G\_5\_5\_10\_75 & 934.2 & 5 & 1.4 &  & 934.2 & 5 & 1.1 &  & 934.2 & 5 & \textbf{0.0} &  & 934.2 & 5 & 0.1 &  & 934.2 & 5 & 1.8 &  \\ \hline
  G\_7\_7\_10\_25 & 712.4 & 5 & 1.5 &  & 712.4 & 5 & 1.2 &  & 712.4 & 5 & \textbf{0.3} &  & 712.4 & 5 & 0.6 &  & 712.4 & 5 & 2.1 &  \\ 
  G\_7\_7\_10\_50 & 1324.2 & 5 & 1.4 &  & 1324.2 & 5 & 1.1 &  & 1324.2 & 5 & \textbf{0.2} &  & 1324.2 & 5 & 0.3 &  & 1324.2 & 5 & 2.0 &  \\ 
  G\_7\_7\_10\_75 & 1998.6 & 5 & 1.5 &  & 1998.6 & 5 & 1.2 &  & 1998.6 & 5 & \textbf{0.2} &  & 1998.6 & 5 & 0.4 &  & 1998.6 & 5 & 2.1 &  \\ \hline
  G\_9\_9\_10\_25 & 1180.8 & 5 & 5.9 &  & 1180.8 & 5 & \textbf{1.5} &  & 1180.8 & 5 & \textbf{1.5} &  & 1180.8 & 5 & 11.0 &  & 1180.8 & 5 & 3.5 &  \\ 
  G\_9\_9\_10\_50 & 2192.2 & 5 & 2.3 &  & 2192.2 & 5 & \textbf{1.3} &  & 2192.2 & 5 & 1.4 &  & 2192.2 & 5 & 1.9 &  & 2192.2 & 5 & 6.4 &  \\ 
  G\_9\_9\_10\_75 & 3452.2 & 5 & 2.0 &  & 3452.2 & 5 & 1.2 &  & 3452.2 & 5 & \textbf{0.9} &  & 3452.2 & 5 & 1.4 &  & 3452.2 & 5 & 2.8 &  \\ 
   \hline
    Average & 1420.4 &  & 2.1 &  & 1420.4 &  & 1.2 &  & 1420.4 &  & 0.5 &  & 1420.4 &  & 1.8 &  & 1420.4 &  & 2.7 &  \\ 
  Total &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  \\ \hline
\end{tabular}
\end{table}



\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations with warm start for the small non-square grid instances.}\label{tab:gridnqinitsol}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
GNQ\_8\_3\_10\_25 & 319.2 & 5 & 1.4 &  & 319.2 & 5 & 1.1 &  & 319.2 & 5 & \textbf{0.0} &  & 319.2 & 5 & 0.1 &  & 319.2 & 5 & 1.8 &  \\ 
  GNQ\_8\_3\_10\_50 & 579.2 & 5 & 1.4 &  & 579.2 & 5 & 1.1 &  & 579.2 & 5 & \textbf{0.1} &  & 579.2 & 5 & \textbf{0.1} &  & 579.2 & 5 & 1.8 &  \\ 
  GNQ\_8\_3\_10\_75 & 838.0 & 5 & 1.3 &  & 838.0 & 5 & 1.1 &  & 838.0 & 5 & \textbf{0.0} &  & 838.0 & 5 & 0.1 &  & 838.0 & 5 & 1.6 &  \\ \hline
  GNQ\_9\_6\_10\_25 & 786.8 & 5 & 1.7 &  & 786.8 & 5 & 1.2 &  & 786.8 & 5 & \textbf{0.2} &  & 786.8 & 5 & 2.0 &  & 786.8 & 5 & 1.9 &  \\ 
  GNQ\_9\_6\_10\_50 & 1438.6 & 5 & 1.5 &  & 1438.6 & 5 & 1.2 &  & 1438.6 & 5 & \textbf{0.3} &  & 1438.6 & 5 & 0.7 &  & 1438.6 & 5 & 2.1 &  \\ 
  GNQ\_9\_6\_10\_75 & 2195.6 & 5 & 1.5 &  & 2195.6 & 5 & 1.2 &  & 2195.6 & 5 & \textbf{0.3} &  & 2195.6 & 5 & 0.6 &  & 2195.6 & 5 & 2.2 &  \\ \hline
  GNQ\_12\_6\_10\_25 & 1071.2 & 5 & 2.5 &  & 1071.2 & 5 & 1.5 &  & 1071.2 & 5 & \textbf{1.2} &  & 1071.2 & 5 & 6.7 &  & 1071.2 & 5 & 11.9 &  \\ 
  GNQ\_12\_6\_10\_50 & 1944.2 & 5 & 1.8 &  & 1944.2 & 5 & 1.2 &  & 1944.2 & 5 & \textbf{1.0} &  & 1944.2 & 5 & 2.2 &  & 1944.2 & 5 & 4.0 &  \\ 
  GNQ\_12\_6\_10\_75 & 3022.4 & 5 & 1.6 &  & 3022.4 & 5 & 1.2 &  & 3022.4 & 5 & \textbf{0.7} &  & 3022.4 & 5 & 1.9 &  & 3022.4 & 5 & 3.5 &  \\ 
   \hline
   Average & 1355.0 &  & 1.6 &  & 1355.0 &  & 1.2 &  & 1355.0 &  & 0.4 &  & 1355.0 &  & 1.6 &  & 1355.0 &  & 3.4 &  \\ 
  Total &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  \\ 
   \hline
\end{tabular}
\end{table}


\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations with warm start for the small hypercube instances.}\label{tab:ipercubeinitsol}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
I\_4\_10\_25 & 147.0 & 5 & 1.4 &  & 147.0 & 5 & 1.1 &  & 147.0 & 5 & \textbf{0.0} &  & 147.0 & 5 & 0.1 &  & 147.0 & 5 & 1.8 &  \\ 
  I\_4\_10\_50 & 289.4 & 5 & 1.4 &  & 289.4 & 5 & 1.1 &  & 289.4 & 5 & \textbf{0.0} &  & 289.4 & 5 & \textbf{0.0} &  & 289.4 & 5 & 1.8 &  \\ 
  I\_4\_10\_75 & 344.0 & 5 & 1.4 &  & 344.0 & 5 & 1.1 &  & 344.0 & 5 & \textbf{0.0} &  & 344.0 & 5 & \textbf{0.0} &  & 344.0 & 5 & 1.8 &  \\ \hline
  I\_5\_10\_25 & 278.4 & 5 & 2.2 &  & 278.4 & 5 & 1.3 &  & 278.4 & 5 & 0.8 &  & 278.4 & 5 & \textbf{0.7} &  & 278.4 & 5 & 2.7 &  \\ 
  I\_5\_10\_50 & 545.0 & 5 & 1.5 &  & 545.0 & 5 & 1.2 &  & 545.0 & 5 & \textbf{0.2} &  & 545.0 & 5 & \textbf{0.2} &  & 545.0 & 5 & 1.9 &  \\ 
  I\_5\_10\_75 & 787.4 & 5 & 1.5 &  & 787.4 & 5 & 1.2 &  & 787.4 & 5 & \textbf{0.1} &  & 787.4 & 5 & \textbf{0.1} &  & 787.4 & 5 & 1.9 &  \\ \hline
  I\_6\_10\_25 & 527.2 & 2 & 2296.9 & 2.0 & 527.2 & 5 & \textbf{22.6} &  & 527.2 & 5 & 60.7 &  & 527.2 & 5 & 66.3 &  & 527.2 & 5 & 1764.0 &  \\ 
  I\_6\_10\_50 & 975.6 & 5 & 19.6 &  & 975.6 & 5 & \textbf{2.7} &  & 975.6 & 5 & 4.8 &  & 975.6 & 5 & 4.1 &  & 975.6 & 5 & 45.8 &  \\ 
  I\_6\_10\_75 & 1250.8 & 5 & 7.1 &  & 1250.8 & 5 & 1.4 &  & 1250.8 & 5 & 1.0 &  & 1250.8 & 5 & \textbf{0.7} &  & 1250.8 & 5 & 3.2 &  \\ 
   \hline
     Average & 571.6 &  & 259.2 & 2.0 & 571.6 &  & 3.7 &  & 571.6 &  & 7.5 &  & 571.6 &  & 8.0 &  & 571.6 &  & 202.7 &  \\ 
  Total &  & 42 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  \\ 
   \hline
\end{tabular}
\end{table}


\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations with warm start for the small toroidal instances.}\label{tab:toroinitsol}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
T\_5\_5\_10\_25 & 232.8 & 5 & 1.4 &  & 232.8 & 5 & 1.1 &  & 232.8 & 5 & \textbf{0.1} &  & 232.8 & 5 & \textbf{0.1} &  & 232.8 & 5 & 1.8 &  \\ 
  T\_5\_5\_10\_50 & 357.2 & 5 & 1.4 &  & 357.2 & 5 & 1.2 &  & 357.2 & 5 & \textbf{0.0} &  & 357.2 & 5 & 0.1 &  & 357.2 & 5 & 1.8 &  \\ 
  T\_5\_5\_10\_75 & 448.6 & 5 & 1.4 &  & 448.6 & 5 & 1.1 &  & 448.6 & 5 & \textbf{0.0} &  & 448.6 & 5 & 0.1 &  & 448.6 & 5 & 1.8 &  \\ \hline
  T\_7\_7\_10\_25 & 471.2 & 5 & 4.6 &  & 471.2 & 5 & 1.3 &  & 471.2 & 5 & \textbf{0.5} &  & 471.2 & 5 & 0.7 &  & 471.2 & 5 & 2.2 &  \\ 
  T\_7\_7\_10\_50 & 734.6 & 5 & 1.7 &  & 734.6 & 5 & 1.3 &  & 734.6 & 5 & \textbf{0.3} &  & 734.6 & 5 & 0.4 &  & 734.6 & 5 & 2.1 &  \\ 
  T\_7\_7\_10\_75 & 912.4 & 5 & 1.6 &  & 912.4 & 5 & 1.2 &  & 912.4 & 5 & \textbf{0.3} &  & 912.4 & 5 & 0.4 &  & 912.4 & 5 & 2.2 &  \\ \hline
  T\_9\_9\_10\_25 & 730.0 & 0 &  & 1.7 & 730.0 & 5 & 10.2 &  & 730.0 & 5 & 5.0 &  & 730.0 & 5 & 17.9 &  & 730.0 & 5 & \textbf{4.0} &  \\ 
  T\_9\_9\_10\_50 & 1130.4 & 5 & 41.4 &  & 1130.4 & 5 & 1.6 &  & 1130.4 & 5 & \textbf{1.0} &  & 1130.4 & 5 & 1.4 &  & 1130.4 & 5 & 3.6 &  \\ 
  T\_9\_9\_10\_75 & 1478.6 & 5 & 12.7 &  & 1478.6 & 5 & 1.5 &  & 1478.6 & 5 & \textbf{1.1} &  & 1478.6 & 5 & 1.2 &  & 1478.6 & 5 & 3.6 &  \\ 
   \hline
    Average & 721.8 &  & 8.3 & 1.7 & 721.8 &  & 2.3 &  & 721.8 &  & 0.9 &  & 721.8 &  & 2.5 &  & 721.8 &  & 2.6 &  \\ 
  Total &  & 40 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  \\ 
   \hline
\end{tabular}
\end{table}




\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations with warm start for the small random instances.}\label{tab:randominitsol}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
R\_25\_33\_10\_25 & 317.2 & 5 & 1.4 &  & 317.2 & 5 & 1.1 &  & 317.2 & 5 & \textbf{0.0} &  & 317.2 & 5 & 0.1 &  & 317.2 & 5 & 1.8 &  \\ 
  R\_25\_33\_10\_50 & 525.8 & 5 & 1.4 &  & 525.8 & 5 & 1.1 &  & 525.8 & 5 & \textbf{0.0} &  & 525.8 & 5 & 0.1 &  & 525.8 & 5 & 1.8 &  \\ 
  R\_25\_33\_10\_75 & 702.8 & 5 & 1.4 &  & 702.8 & 5 & 1.1 &  & 702.8 & 5 & \textbf{0.0} &  & 702.8 & 5 & 0.1 &  & 702.8 & 5 & 1.4 &  \\ \hline
  R\_25\_69\_10\_25 & 243.0 & 5 & 1.4 &  & 243.0 & 5 & 1.2 &  & 243.0 & 5 & 0.2 &  & 243.0 & 5 & \textbf{0.1} &  & 243.0 & 5 & 1.8 &  \\ 
  R\_25\_69\_10\_50 & 389.8 & 5 & 1.5 &  & 389.8 & 5 & 1.2 &  & 389.8 & 5 & 0.2 &  & 389.8 & 5 & \textbf{0.1} &  & 389.8 & 5 & 1.9 &  \\ 
  R\_25\_69\_10\_75 & 597.2 & 5 & 1.5 &  & 597.2 & 5 & 1.2 &  & 597.2 & 5 & \textbf{0.1} &  & 597.2 & 5 & \textbf{0.1} &  & 597.2 & 5 & 1.9 &  \\ \hline
  R\_25\_204\_10\_25 & 106.8 & 5 & 1.7 &  & 106.8 & 5 & 1.5 &  & 106.8 & 5 & 1.7 &  & 106.8 & 5 & \textbf{0.9} &  & 106.8 & 5 & 2.3 &  \\ 
  R\_25\_204\_10\_50 & 193.0 & 5 & 1.6 &  & 193.0 & 5 & 1.4 &  & 193.0 & 5 & 1.3 &  & 193.0 & 5 & \textbf{0.7} &  & 193.0 & 5 & 2.3 &  \\ 
  R\_25\_204\_10\_75 & 312.2 & 5 & 1.6 &  & 312.2 & 5 & 1.4 &  & 312.2 & 5 & 1.3 &  & 312.2 & 5 & \textbf{0.7} &  & 312.2 & 5 & 2.2 &  \\ \hline
  R\_50\_85\_10\_25 & 583.2 & 5 & 2.1 &  & 583.2 & 5 & 1.2 &  & 583.2 & 5 & \textbf{0.1} &  & 583.2 & 5 & 0.4 &  & 583.2 & 5 & 1.9 &  \\ 
  R\_50\_85\_10\_50 & 957.2 & 5 & 1.8 &  & 957.2 & 5 & 1.2 &  & 957.2 & 5 & \textbf{0.2} &  & 957.2 & 5 & 0.3 &  & 957.2 & 5 & 2.1 &  \\ 
  R\_50\_85\_10\_75 & 1229.8 & 5 & 1.6 &  & 1229.8 & 5 & 1.2 &  & 1229.8 & 5 & \textbf{0.2} &  & 1229.8 & 5 & 0.3 &  & 1229.8 & 5 & 2.0 &  \\ \hline
  R\_50\_232\_10\_25 & 355.2 & 5 & 77.5 &  & 355.2 & 5 & \textbf{2.0} &  & 355.2 & 5 & 5.3 &  & 355.2 & 5 & 3.0 &  & 355.2 & 5 & 4.0 &  \\ 
  R\_50\_232\_10\_50 & 657.2 & 5 & 28.7 &  & 657.2 & 5 & \textbf{1.7} &  & 657.2 & 5 & 4.7 &  & 657.2 & 5 & 2.2 &  & 657.2 & 5 & 4.2 &  \\ 
  R\_50\_232\_10\_75 & 889.6 & 5 & 27.5 &  & 889.6 & 5 & \textbf{1.7} &  & 889.6 & 5 & 4.1 &  & 889.6 & 5 & 2.2 &  & 889.6 & 5 & 4.1 &  \\ \hline
  R\_50\_784\_10\_25 & 146.4 & 5 & 231.0 &  & 146.4 & 5 & \textbf{8.4} &  & 146.4 & 5 & 53.8 &  & 146.4 & 5 & 32.3 &  & 146.4 & 5 & 9.8 &  \\ 
  R\_50\_784\_10\_50 & 278.2 & 5 & 172.1 &  & 278.2 & 5 & \textbf{8.5} &  & 278.2 & 5 & 32.6 &  & 278.2 & 5 & 15.9 &  & 278.2 & 5 & 9.0 &  \\ 
  R\_50\_784\_10\_75 & 415.6 & 5 & 133.3 &  & 415.6 & 5 & \textbf{7.8} &  & 415.6 & 5 & 31.2 &  & 415.6 & 5 & 13.8 &  & 415.6 & 5 & 8.2 &  \\ \hline
  R\_75\_157\_10\_25 & 792.0 & 5 & 804.8 &  & 792.0 & 5 & 3.1 &  & 792.0 & 5 & \textbf{1.0} &  & 792.0 & 5 & 2.8 &  & 792.0 & 5 & 3.0 &  \\ 
  R\_75\_157\_10\_50 & 1250.6 & 5 & 195.9 &  & 1250.6 & 5 & 2.2 &  & 1250.6 & 5 & \textbf{0.9} &  & 1250.6 & 5 & 1.1 &  & 1250.6 & 5 & 3.4 &  \\ 
  R\_75\_157\_10\_75 & 1870.6 & 5 & 62.8 &  & 1870.6 & 5 & 1.7 &  & 1870.6 & 5 & 1.2 &  & 1870.6 & 5 & \textbf{0.9} &  & 1870.6 & 5 & 5.8 &  \\ \hline
  R\_75\_490\_10\_25 & 461.8 & 0 &  & 13.7 & 461.8 & 5 & \textbf{12.5} &  & 461.8 & 5 & 129.1 &  & 461.8 & 5 & 69.2 &  & 461.8 & 5 & 41.4 &  \\ 
  R\_75\_490\_10\_50 & 797.4 & 0 &  & 15.6 & 797.4 & 5 & \textbf{20.1} &  & 797.4 & 5 & 167.6 &  & 797.4 & 5 & 70.7 &  & 797.4 & 5 & 56.7 &  \\ 
  R\_75\_490\_10\_75 & 1233.4 & 0 &  & 9.8 & 1233.4 & 5 & \textbf{6.3} &  & 1233.4 & 5 & 81.5 &  & 1233.4 & 5 & 32.2 &  & 1233.4 & 5 & 35.4 &  \\ \hline
  R\_75\_1739\_10\_25 & 158.4 & 0 &  & 47.2 & 158.4 & 5 & \textbf{133.0} &  & 158.4 & 5 & 808.2 &  & 158.4 & 5 & 372.0 &  & 158.4 & 5 & 138.7 &  \\ 
  R\_75\_1739\_10\_50 & 300.4 & 0 &  & 38.3 & 300.4 & 5 & \textbf{100.0} &  & 300.4 & 5 & 690.5 &  & 300.4 & 5 & 331.5 &  & 300.4 & 5 & 103.4 &  \\ 
  R\_75\_1739\_10\_75 & 458.2 & 0 &  & 36.2 & 458.2 & 5 & 97.7 &  & 458.2 & 5 & 695.4 &  & 458.2 & 5 & 298.6 &  & 458.2 & 5 & \textbf{91.5} &  \\ 
   \hline
       Average & 600.9 &  & 83.5 & 26.8 & 600.9 &  & 15.6 &  & 600.9 &  & 100.5 &  & 600.9 &  & 46.4 &  & 600.9 &  & 20.1 &  \\ 
  Total &  & 105 &  &  &  & 135 &  &  &  & 135 &  &  &  & 135 &  &  &  & 135 &  &  \\ 
   \hline
\end{tabular}
\end{table}

\end{landscape}

The plots in Figure~\ref{fig:comparison-small-instances} compare the average computation times over all individual small instances in each class for each formulation, (a) using the standalone formulations and (b) running with feasible warm starts generated by the matheuristic MILS$^+$-$mtz$.
%The plots show that TCYC is the best performing formulation for several classes. 
The plots show that TCYC is, overall, the best performing formulation for this set of instances as it takes lower average computation times to solve the instances to optimality. Note that TCYC outperforms all other formulations for hypercube and random graphs. 
They also illustrate that formulation DCUT is the mostly benefited by the warm starts.

%The plots show that TCYC is the best performing formulation for several classes. They also illustrate that formulation DCUT is the mostly benefited by the warm starts, but mainly the average times show that almost all instances could be solved to optimality below the time limit of 3600 seconds.}

\begin{figure}[ht!]
\begin{center}
    \begin{tabular}{cc}
    \includegraphics[width=0.5\textwidth]{cputime_Small_original.pdf} & \includegraphics[width=0.5\textwidth]{cputime_Small_initialsolution.pdf}\\
(a) Standalone formulations & (b) Running with warm starts
%  (a) Aggregated results for small instances  & (b) Aggregated results for small instances\\    running as standalone formulations & with warm starts
\end{tabular}
\end{center}
\caption{Average computation times in seconds over all small instances in each class for each formulation, (a) first using the standalone formulations, and (b) then running with feasible warm starts generated by the matheuristic MILS$^+$-$mtz$. For each instance, the computation time considered in the averages is either the time to prove optimality (if less than the imposed time limit of 3600 seconds) or this imposed time limit.}
\label{fig:comparison-small-instances}
\end{figure}

\subsection{Large instances}
\label{sec:largeinstances}


Tables~\ref{tab:gridlarge}-\ref{tab:randlargeinitsol} summarize the results for the large instances, 
with Tables~\ref{tab:gridlarge}-\ref{tab:randlarge} corresponding to the formulations as standalone approaches and Tables~\ref{tab:gridlargeinitsol}-\ref{tab:randlargeinitsol} to the formulations when offered warm starts.
Tables~\ref{tab:gridlarge}~and~\ref{tab:gridnqlarge} show that for the large grid instances, FLOW clearly outperformed the other approaches, achieving 50 and 54 solved instances for the square and nonsquare grid instances, respectively.
Table~\ref{tab:ipercubelarge} displays that, for the large hypercube instances, MTZ outperforms the other approaches in terms of number of solutions solved to optimality. This is partly due to the fact that the solver is able to generate good quality feasible solutions earlier in the search process.
Table~\ref{tab:torolarge} shows that, for the large toroidal instances, FLOW outperformed the other approaches when it comes to the number of solved instances, closely followed by MTZ. 
Table~\ref{tab:randlarge} exhibits that, for the large random instances, MTZ, TCYC, and DCUT solved nearly the same number of instances with TCYC presenting much lower average times. Note that TCYC performed considerably better for the instances with 100 nodes. For very large random instance groups, the open gap was usually very high, with DCUT often achieving the lowest values.  
%Overall, when a good quality solution is not available, FLOW and MTZ show themselves to be more viable to be used in a commercial solver as standalone procedure.


Tables~\ref{tab:gridlargeinitsol}-\ref{tab:randlargeinitsol} show the results for the large instances when a good quality initial feasible solution obtained by the matheuristic of \citeA{MelQueRib21} is offered to the solver. 
Tables~\ref{tab:gridlargeinitsol}~and~\ref{tab:gridnqlargeinitsol} reveal that, for the large grid instances, considerable reductions in the average open gaps were achieved for CYC, TCYC and DCUT when compared to the standalone formulation.
Table~\ref{tab:ipercubelargeinitsol} unveils that, for the large hypercube instances, considerable gains in the gaps can be observed for CYC, TCYC and DCUT. Furthermore, the use of good quality warm starts turns DCUT into a very competitive approach for proving optimality of the instances.
Table~\ref{tab:torolargeinitsol} shows that, for the large toroidal instances, again, warm starts allowed a considerable reduction in the average open gaps for CYC, TCYC, and DCUT.
Table~\ref{tab:randlargeinitsol} displays that, for the large random instances, TCYC presented outstanding results when compared to the other approaches, especially on the average time to solve instances to optimality. Even though MTZ proved optimality of one additional instance, the average times achieved by TCYC and DCUT were much lower. We note, though, that for the larger instances, the open gap is still large, even for the best performing approaches.




\begin{landscape}




\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations for the large square grid instances.}\label{tab:gridlarge}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
G\_10\_10\_10\_25 & 1504.0 & 5 & 128.5 &  & 1504.0 & 5 & \textbf{3.4} &  & 1504.0 & 5 & 4.5 &  & 1504.0 & 5 & 22.7 &  & 1504.0 & 5 & 795.4 &  \\ 
  G\_10\_10\_10\_50 & 2722.0 & 5 & 5.0 &  & 2722.0 & 5 & \textbf{1.5} &  & 2722.0 & 5 & 5.0 &  & 2722.0 & 5 & 10.7 &  & 2722.0 & 5 & 787.3 &  \\ 
  G\_10\_10\_10\_75 & 4307.6 & 5 & 7.6 &  & 4307.6 & 5 & \textbf{2.5} &  & 4307.6 & 5 & 5.7 &  & 4307.6 & 5 & 14.3 &  & 4307.6 & 5 & 1602.4 &  \\ \hline
  G\_14\_14\_10\_25 & 2989.8 & 0 &  & 3.8 & 2996.2 & \textbf{5} & 1370.3 &  & 2996.2 & \textbf{5} & 64.8 &  & 2996.2 & 4 & 1632.1 & 0.1 & 1246.0 & 0 &  & 58.6 \\ 
  G\_14\_14\_10\_50 & 5487.4 & 0 &  & 1.8 & 5489.0 & 4 & 55.5 & 0.1 & 5489.0 & \textbf{5} & 166.7 &  & 5489.0 & \textbf{5} & 359.7 &  & 953.8 & 0 &  & 82.7 \\ 
  G\_14\_14\_10\_75 & 8794.6 & 0 &  & 3.1 & 8807.8 & 1 & 149.8 & 0.3 & 8808.2 & \textbf{5} & 129.8 &  & 8808.2 & 3 & 472.5 & 0.2 & 3950.8 & 0 &  & 55.4 \\ \hline 
  G\_17\_17\_10\_25 & 4387.0 & 0 &  & 5.8 & 4427.2 & 0 &  & 0.2 & 4427.6 & \textbf{4} & 387.3 & 0.0 & 4427.6 & 1 & 2691.5 & 0.1 & 89.8 & 0 &  & 98.0 \\ 
  G\_17\_17\_10\_50 & 8144.2 & 0 &  & 3.5 & 8185.6 & \textbf{5} & 911.8 &  & 8185.6 & 4 & 669.0 & 0.1 & 8185.6 & 4 & 1281.0 & 0.1 & 192.6 & 0 &  & 97.6 \\ 
  G\_17\_17\_10\_75 & 13125.0 & 0 &  & 4.0 & 13151.2 & 1 & 2497.6 & 0.4 & 13155.2 & \textbf{5} & 786.6 &  & 13155.2 & 1 & 676.6 & 0.1 & 86.6 & 0 &  & 99.3 \\ \hline
  G\_20\_20\_10\_25 & 5973.4 & 0 &  & 8.9 & 6154.4 & 0 &  & 0.6 & 6172.0 & \textbf{2} & 2280.2 & 0.1 & 6173.8 & 0 &  & 0.1 & 404.8 & 0 &  & 93.5 \\ 
  G\_20\_20\_10\_50 & 11117.6 & 0 &  & 5.8 & 11343.0 & 0 &  & 0.3 & 11345.0 & \textbf{2} & 2933.0 & 0.1 & 11345.6 & 0 &  & 0.1 & 37.2 & 0 &  & 99.7 \\ 
  G\_20\_20\_10\_75 & 18058.6 & 0 &  & 6.3 & 18388.8 & 0 &  & 0.6 & 18408.8 & \textbf{2} & 1623.5 & 0.0 & 18408.6 & 0 &  & 0.1 & 79.2 & 0 &  & 99.6 \\ \hline
  G\_23\_23\_10\_25 & 7790.8 & 0 &  & 10.5 & 8099.2 & 0 &  & 1.2 & 8175.8 & \textbf{1} & 668.3 & 0.1 & 8176.0 & 0 &  & 0.1 & 858.0 & 0 &  & 89.5 \\ 
  G\_23\_23\_10\_50 & 14762.8 & 0 &  & 6.9 & 15194.2 & 0 &  & 0.4 & 15197.6 & 0 &  & \textbf{0.1} & 15195.6 & 0 &  & 0.2 & 151.4 & 0 &  & 99.0 \\ 
  G\_23\_23\_10\_75 & 23476.0 & 0 &  & 8.9 & 24348.0 & 0 &  & 1.1 & 24508.8 & 0 &  & \textbf{0.1} & 24498.4 & 0 &  & 0.2 & 504.0 & 0 &  & 97.9 \\ 
   \hline
     Average & 8842.7 &  & 47.1 & 5.8 & 9007.9 &  & 624.1 & 0.5 & 9026.9 &  & 748.0 & 0.1 & 9026.2 &  & 795.7 & 0.1 & 1139.2 &  & 1061.7 & 89.2 \\ 
  Total &  & 15 &  &  &  & 31 &  &  &  & 50 &  &  &  & 33 &  &  &  & 15 &  &  \\ 
   \hline
\end{tabular}
\end{table}


\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations for the large non-square grid instances.}\label{tab:gridnqlarge}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
GNQ\_13\_7\_10\_25 & 1347.8 & 5 & 20.2 &  & 1347.8 & 5 & \textbf{2.0} &  & 1347.8 & 5 & 5.6 &  & 1347.8 & 5 & 27.8 &  & 1345.4 & 3 & 592.2 & 0.9 \\ 
  GNQ\_13\_7\_10\_50 & 2456.6 & 5 & 2.4 &  & 2456.6 & 5 & \textbf{1.2} &  & 2456.6 & 5 & 1.3 &  & 2456.6 & 5 & 2.1 &  & 2456.6 & 5 & 362.3 &  \\ 
  GNQ\_13\_7\_10\_75 & 3876.6 & 5 & 4.1 &  & 3876.6 & 5 & \textbf{1.6} &  & 3876.6 & 5 & 3.8 &  & 3876.6 & 5 & 16.4 &  & 3876.6 & 5 & 410.4 &  \\ \hline
  GNQ\_18\_11\_10\_25 & 3002.8 & 0 &  & 3.2 & 3005.0 & 4 & 294.5 & 0.2 & 3005.0 & \textbf{5} & 102.0 &  & 3005.0 & 4 & 1141.9 & 0.2 & 1330.6 & 0 &  & 55.6 \\ 
  GNQ\_18\_11\_10\_50 & 5504.6 & 0 &  & 2.4 & 5510.2 & 5 & 189.1 &  & 5510.2 & 5 & \textbf{160.4} &  & 5510.2 & 5 & 354.7 &  & 1567.6 & 0 &  & 71.4 \\ 
  GNQ\_18\_11\_10\_75 & 8824.0 & 0 &  & 2.7 & 8829.2 & 3 & 1065.3 & 0.4 & 8829.6 & \textbf{5} & 206.3 &  & 8829.6 & 4 & 809.2 & 0.2 & 3761.0 & 0 &  & 57.4 \\ \hline
  GNQ\_23\_13\_10\_25 & 4533.8 & 0 &  & 6.8 & 4608.8 & 0 &  & 0.2 & 4608.8 & \textbf{5} & 484.8 &  & 4609.2 & 0 &  & 0.1 & 1279.8 & 0 &  & 72.3 \\ 
  GNQ\_23\_13\_10\_50 & 8428.6 & 0 &  & 3.5 & 8453.2 & 2 & 2382.5 & 0.3 & 8455.2 & \textbf{4} & 1038.1 & 0.1 & 8455.2 & \textbf{4} & 1693.3 & 0.1 & 30.6 & 0 &  & 99.6 \\ 
  GNQ\_23\_13\_10\_75 & 13532.4 & 0 &  & 4.2 & 13597.6 & 0 &  & 0.4 & 13599.4 & \textbf{4} & 961.1 & 0.1 & 13599.4 & 1 & 1482.1 & 0.1 & 65.4 & 0 &  & 99.5 \\ \hline
  GNQ\_26\_15\_10\_25 & 5866.8 & 0 &  & 7.9 & 5998.4 & 0 &  & 0.4 & 6005.8 & \textbf{3} & 1077.6 & 0.0 & 6005.8 & 0 &  & 0.1 & 563.8 & 0 &  & 90.6 \\ 
  GNQ\_26\_15\_10\_50 & 10971.2 & 0 &  & 4.6 & 11098.4 & 1 & 951.6 & 0.3 & 11099.0 & \textbf{3} & 2736.7 & 0.1 & 11099.0 & 1 & 1842.5 & 0.1 & 620.6 & 0 &  & 94.4 \\ 
  GNQ\_26\_15\_10\_75 & 17554.4 & 0 &  & 6.3 & 17887.0 & 0 &  & 0.5 & 17906.4 & \textbf{4} & 1349.0 & 0.0 & 17906.4 & 1 & 2292.7 & 0.1 & 129.8 & 0 &  & 99.3 \\ \hline
  GNQ\_29\_17\_10\_25 & 7317.8 & 0 &  & 10.0 & 7608.8 & 0 &  & 0.5 & 7626.0 & \textbf{1} & 938.7 & 0.1 & 7626.4 & 0 &  & 0.1 & 906.6 & 0 &  & 88.1 \\ 
  GNQ\_29\_17\_10\_50 & 13695.0 & 0 &  & 6.7 & 14052.4 & 0 &  & 0.5 & 14066.8 & 0 &  & \textbf{0.1} & 14062.0 & 0 &  & 0.2 & 275.4 & 0 &  & 98.1 \\ 
  GNQ\_29\_17\_10\_75 & 22145.0 & 0 &  & 7.2 & 22677.0 & 0 &  & 0.9 & 22763.8 & 0 &  & \textbf{0.1} & 22763.4 & 0 &  & 0.2 & 842.8 & 0 &  & 96.3 \\ 
   \hline
   Average & 8603.8 &  & 8.9 & 5.5 & 8733.8 &  & 611.0 & 0.4 & 8743.8 &  & 697.3 & 0.1 & 8743.5 &  & 966.3 & 0.2 & 1270.2 &  & 455.0 & 78.7 \\ 
  Total &  & 15 &  &  &  & 30 &  &  &  & 54 &  &  &  & 35 &  &  &  & 13 &  &  \\ 
   \hline
\end{tabular}
\end{table}


\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations for the large hypercube instances.}\label{tab:ipercubelarge}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
I\_7\_10\_25 & 992.2 & 0 &  & 17.1 & 1037.4 & \textbf{1} & 3530.6 & 1.9 & 1037.4 & 0 &  & 1.9 & 1037.4 & \textbf{1} & 2510.8 & 1.5 & 1019.6 & 0 &  & 5.0 \\ 
  I\_7\_10\_50 & 1908.6 & 0 &  & 7.7 & 1935.6 & 5 & 293.3 &  & 1935.6 & 5 & 315.7 &  & 1935.6 & 5 & \textbf{147.1} &  & 1919.0 & 3 & 143.9 & 3.8 \\ 
  I\_7\_10\_75 & 2532.8 & 0 &  & 3.5 & 2533.6 & 5 & 34.7 &  & 2533.6 & 5 & 18.6 &  & 2533.6 & 5 & \textbf{9.3} &  & 2533.6 & 5 & 117.1 &  \\ \hline
  I\_8\_10\_25 & 1954.6 & 0 &  & 21.7 & 2032.2 & 0 &  & 4.3 & 2046.8 & 0 &  & 3.9 & 2064.4 & 0 &  & 2.3 & 1018.0 & 0 &  & 52.3 \\ 
  I\_8\_10\_50 & 3456.8 & 0 &  & 18.8 & 3680.2 & 0 &  & 4.2 & 3704.6 & 0 &  & 2.7 & 3710.2 & 0 &  & \textbf{1.7} & 3677.2 & 0 &  & 3.9 \\ 
  I\_8\_10\_75 & 4258.2 & 0 &  & 22.3 & 4856.2 & 0 &  & 3.7 & 4945.6 & 3 & 2525.9 & 1.0 & 4948.4 & \textbf{4} & 728.5 & 0.5 & 4919.8 & 0 &  & 1.5 \\ \hline
  I\_9\_10\_25 & 0.0 & 0 &  & 100.0 & 3908.6 & 0 &  & 6.5 & 3910.4 & 0 &  & 6.5 & 3925.8 & 0 &  & \textbf{5.9} & 1397.8 & 0 &  & 66.9 \\ 
  I\_9\_10\_50 & 3926.4 & 0 &  & 56.1 & 2949.4 & 0 &  & 62.5 & 7252.0 & 0 &  & 5.1 & 7309.2 & 0 &  & \textbf{4.1} & 4300.4 & 0 &  & 43.0 \\ 
  I\_9\_10\_75 & 1172.4 & 0 &  & 89.5 & 0.0 & 0 &  & 100.0 & 9244.2 & 0 &  & 3.7 & 9305.0 & 0 &  & \textbf{2.7} & 5302.2 & 0 &  & 45.1 \\ \hline 
  Average & 2244.7 &  &  & 37.4 & 2548.1 &  & 1286.2 & 26.2 & 4067.8 &  & 953.4 & 3.5 & 4085.5 &  & 848.9 & 2.7 & 2898.6 &  & 130.5 & 27.7 \\ 
  Total &  & 0 &  &  &  & 11 &  &  &  & 13 &  &  &  & 15 &  &  &  & 8 &  &  \\ 
   \hline
\end{tabular}
\end{table}


% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Sat Aug 29 13:41:23 2020
\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations for the large toroidal instances.}\label{tab:torolarge}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
T\_10\_10\_10\_25 & 943.2 & 0 &  & 3.3 & 946.2 & 5 & 25.3 &  & 946.2 & 5 & \textbf{13.5} &  & 946.2 & 5 & 32.4 &  & 946.2 & 5 & 415.5 &  \\ 
  T\_10\_10\_10\_50 & 1350.4 & 5 & 1289.7 &  & 1350.4 & 5 & 6.1 &  & 1350.4 & 5 & \textbf{4.2} &  & 1350.4 & 5 & 15.4 &  & 1349.4 & 4 & 707.5 & 0.9 \\ 
  T\_10\_10\_10\_75 & 1778.0 & 5 & 76.3 &  & 1778.0 & 5 & 3.0 &  & 1778.0 & 5 & \textbf{1.5} &  & 1778.0 & 5 & 1.9 &  & 1766.0 & 4 & 124.6 & 4.2 \\ \hline
  T\_14\_14\_10\_25 & 1803.4 & 0 &  & 6.8 & 1839.4 & 1 & 50.7 & 0.5 & 1840.6 & \textbf{5} & 422.0 &  & 1840.6 & \textbf{5} & 647.7 &  & 1463.8 & 1 & 29.0 & 25.3 \\ 
  T\_14\_14\_10\_50 & 2794.2 & 0 &  & 2.4 & 2801.6 & 3 & 128.8 & 0.4 & 2801.6 & \textbf{5} & 57.4 &  & 2801.6 & \textbf{5} & 87.0 &  & 641.6 & 0 &  & 76.7 \\ 
  T\_14\_14\_10\_75 & 3726.8 & 1 & 824.4 & 1.2 & 3728.2 & 5 & 84.7 &  & 3728.2 & 5 & \textbf{54.7} &  & 3728.2 & 5 & 74.4 &  & 239.0 & 0 &  & 93.7 \\ \hline
  T\_17\_17\_10\_25 & 2625.8 & 0 &  & 9.2 & 2732.4 & 0 &  & 0.8 & 2739.8 & \textbf{2} & 867.5 & 0.2 & 2739.8 & 1 & 518.4 & 0.2 & 100.6 & 0 &  & 96.4 \\ 
  T\_17\_17\_10\_50 & 4052.4 & 0 &  & 4.1 & 4112.2 & 0 &  & 0.3 & 4112.4 & \textbf{5} & 603.2 &  & 4112.4 & \textbf{5} & 644.7 &  & 26.4 & 0 &  & 99.4 \\ 
  T\_17\_17\_10\_75 & 5458.4 & 0 &  & 1.9 & 5477.6 & 2 & 1885.4 & 0.3 & 5477.8 & \textbf{5} & 613.2 &  & 5477.8 & \textbf{5} & 349.7 &  & 25.6 & 0 &  & 99.5 \\ \hline
  T\_20\_20\_10\_25 & 3566.4 & 0 &  & 11.5 & 3729.8 & 0 &  & 2.5 & 3801.4 & \textbf{1} & 3598.0 & 0.2 & 3801.0 & 0 &  & 0.2 & 202.2 & 0 &  & 94.7 \\ 
  T\_20\_20\_10\_50 & 5451.4 & 0 &  & 5.9 & 5605.2 & 0 &  & 0.8 & 5622.2 & \textbf{3} & 1874.8 & 0.1 & 5622.0 & \textbf{3} & 2374.0 & 0.1 & 132.2 & 0 &  & 97.7 \\ 
  T\_20\_20\_10\_75 & 7254.0 & 0 &  & 3.6 & 7376.6 & 0 &  & 0.4 & 7383.8 & \textbf{5} & 1297.7 &  & 7383.8 & 4 & 817.1 & 0.1 & 49.8 & 0 &  & 99.3 \\ \hline
  T\_23\_23\_10\_25 & 4578.8 & 0 &  & 13.9 & 4852.4 & 0 &  & 3.7 & 5002.6 & 0 &  & \textbf{0.4} & 5000.0 & 0 &  & \textbf{0.4} & 35.8 & 0 &  & 99.3 \\ 
  T\_23\_23\_10\_50 & 7160.0 & 0 &  & 8.0 & 7513.0 & 0 &  & 1.0 & 7552.2 & \textbf{1} & 2292.9 & 0.1 & 7551.6 & \textbf{1} & 2584.3 & 0.1 & 31.0 & 0 &  & 99.6 \\ 
  T\_23\_23\_10\_75 & 9858.6 & 0 &  & 4.3 & 10090.0 & 0 &  & 0.7 & 10116.2 & \textbf{2} & 3357.0 & 0.0 & 10116.2 & 1 & 1409.0 & 0.1 & 67.8 & 0 &  & 99.3 \\ 
   \hline
     Average & 4160.1 &  & 730.1 & 5.9 & 4262.2 &  & 312.0 & 1.0 & 4283.6 &  & 1075.5 & 0.2 & 4283.3 &  & 735.1 & 0.2 & 471.8 &  & 319.1 & 77.6 \\ 
  Total &  & 11 &  &  &  & 26 &  &  &  & 54 &  &  &  & 50 &  &  &  & 14 &  &  \\ 
   \hline
\end{tabular}
\end{table}


% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Thu Sep 17 14:46:25 2020
\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations for the large random instances.}\label{tab:randlarge}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
R\_100\_247\_10\_25 & 990.8 & 0 &  & 8.4 & 1004.6 & 5 & 16.5 &  & 1004.6 & 5 & 8.8 &  & 1004.6 & 5 & \textbf{7.7} &  & 1004.6 & 5 & 27.6 &  \\ 
  R\_100\_247\_10\_50 & 1683.0 & 0 &  & 7.0 & 1696.4 & 5 & 88.4 &  & 1696.4 & 5 & \textbf{9.1} &  & 1696.4 & 5 & 12.0 &  & 1696.4 & 5 & 121.7 &  \\ 
  R\_100\_247\_10\_75 & 2440.0 & 0 &  & 5.9 & 2449.2 & 5 & 80.0 &  & 2449.2 & 5 & 8.9 &  & 2449.2 & 5 & \textbf{7.3} &  & 2449.2 & 5 & 56.5 &  \\ \hline
  R\_100\_841\_10\_25 & 456.2 & 0 &  & 33.4 & 492.0 & 5 & \textbf{174.4} &  & 492.0 & 5 & 2387.5 &  & 492.0 & 5 & 874.6 &  & 492.0 & 5 & 1480.3 &  \\ 
  R\_100\_841\_10\_50 & 839.6 & 0 &  & 37.5 & 949.8 & 5 & \textbf{594.3} &  & 948.8 & 3 & 2166.4 & 1.9 & 949.8 & 5 & 1096.3 &  & 949.8 & 5 & 1796.8 &  \\ 
  R\_100\_841\_10\_75 & 1187.6 & 0 &  & 36.7 & 1350.8 & 5 & \textbf{313.3} &  & 1350.8 & 5 & 1852.2 &  & 1350.8 & 5 & 1020.7 &  & 1350.8 & 5 & 1488.8 &  \\ \hline
  R\_100\_3069\_10\_25 & 142.4 & 0 &  & 71.5 & 169.6 & 5 & \textbf{1050.2} &  & 166.6 & 0 &  & 36.0 & 169.6 & 5 & 2826.1 &  & 169.6 & 5 & 1079.6 &  \\ 
  R\_100\_3069\_10\_50 & 258.8 & 0 &  & 71.4 & 326.4 & 5 & 728.1 &  & 315.2 & 1 & 3453.0 & 32.4 & 326.4 & 5 & 2220.8 &  & 326.4 & 5 & \textbf{702.6} &  \\ 
  R\_100\_3069\_10\_75 & 397.4 & 0 &  & 71.0 & 489.8 & 5 & 723.4 &  & 480.4 & 1 & 3305.2 & 29.8 & 489.8 & 5 & 1905.9 &  & 489.8 & 5 & \textbf{622.4} &  \\ \hline
  R\_200\_796\_10\_25 & 788.4 & 0 &  & 65.3 & 1619.8 & 0 &  & 7.7 & 1676.6 & 0 &  & 4.9 & 1681.6 & 0 &  & \textbf{3.3} & 1667.4 & 0 &  & 7.6 \\ 
  R\_200\_796\_10\_50 & 961.2 & 0 &  & 74.3 & 2720.8 & 0 &  & 7.3 & 2818.0 & 0 &  & 4.3 & 2824.0 & 0 &  & \textbf{2.5} & 2735.4 & 0 &  & 10.2 \\ 
  R\_200\_796\_10\_75 & 1721.2 & 0 &  & 64.1 & 3718.4 & 0 &  & 4.5 & 3757.6 & 0 &  & 3.9 & 3764.8 & \textbf{1} & 2903.8 & 2.2 & 3706.0 & 0 &  & 7.5 \\ \hline
  R\_200\_3184\_10\_25 & 264.0 & 0 &  & 82.9 & 569.0 & 0 &  & 39.0 & 593.8 & 0 &  & 41.3 & 613.6 & 0 &  & \textbf{34.5} & 622.4 & 0 &  & 36.1 \\ 
  R\_200\_3184\_10\_50 & 590.6 & 0 &  & 78.9 & 1072.2 & 0 &  & 35.9 & 1122.2 & 0 &  & 39.9 & 1113.2 & 0 &  & \textbf{34.6} & 1113.4 & 0 &  & 40.5 \\ 
  R\_200\_3184\_10\_75 & 668.2 & 0 &  & 83.3 & 1597.8 & 0 &  & \textbf{32.4} & 1656.0 & 0 &  & 37.1 & 1605.0 & 0 &  & 33.2 & 1666.0 & 0 &  & 33.5 \\ \hline
  R\_200\_12139\_10\_25 & 113.8 & 0 &  & 91.1 & 151.0 & 0 &  & 82.5 & 183.0 & 0 &  & 86.1 & 185.8 & 0 &  & 80.5 & 189.2 & 0 &  & \textbf{62.1} \\ 
  R\_200\_12139\_10\_50 & 212.8 & 0 &  & 90.2 & 262.4 & 0 &  & 79.9 & 335.2 & 0 &  & 82.8 & 339.0 & 0 &  & 78.4 & 355.6 & 0 &  & \textbf{56.1} \\ 
  R\_200\_12139\_10\_75 & 304.0 & 0 &  & 89.7 & 292.4 & 0 &  & 85.5 & 471.2 & 0 &  & 83.7 & 483.6 & 0 &  & 77.2 & 489.4 & 0 &  & \textbf{56.0} \\ \hline
  R\_300\_1644\_10\_25 & 525.2 & 0 &  & 81.6 & 1886.6 & 0 &  & 11.5 & 1930.6 & 0 &  & 10.6 & 1948.0 & 0 &  & \textbf{9.4} & 1937.6 & 0 &  & 11.9 \\ 
  R\_300\_1644\_10\_50 & 327.8 & 0 &  & 93.7 & 3273.6 & 0 &  & 17.3 & 3372.0 & 0 &  & 16.1 & 3450.6 & 0 &  & \textbf{13.4} & 3386.0 & 0 &  & 15.8 \\ 
  R\_300\_1644\_10\_75 & 482.2 & 0 &  & 94.2 & 4904.6 & 0 &  & 16.0 & 5110.4 & 0 &  & 13.9 & 5146.6 & 0 &  & \textbf{12.3} & 5058.4 & 0 &  & 17.7 \\ \hline
  R\_300\_7026\_10\_25 & 280.8 & 0 &  & 88.4 & 566.0 & 0 &  & 59.3 & 659.8 & 0 &  & 60.2 & 637.2 & 0 &  & 56.4 & 650.0 & 0 &  & \textbf{55.9} \\ 
  R\_300\_7026\_10\_50 & 459.6 & 0 &  & 90.1 & 1081.4 & 0 &  & 58.4 & 1267.2 & 0 &  & 59.8 & 1270.6 & 0 &  & \textbf{54.5} & 1232.8 & 0 &  & 56.3 \\ 
  R\_300\_7026\_10\_75 & 658.2 & 0 &  & 90.0 & 1675.4 & 0 &  & 55.2 & 1757.4 & 0 &  & 60.6 & 1752.8 & 0 &  & \textbf{55.0} & 1770.0 & 0 &  & 55.1 \\ \hline
  R\_300\_27209\_10\_25 & 116.0 & 0 &  & 94.9 & 0.0 & 0 &  & 100.0 & 0.0 & 0 &  & 100.0 & 184.2 & 0 &  & 90.7 & 187.0 & 0 &  & \textbf{74.9} \\ 
  R\_300\_27209\_10\_50 & 181.4 & 0 &  & 94.8 & 5.8 & 0 &  & 99.7 & 143.6 & 0 &  & 95.9 & 371.2 & 0 &  & 87.8 & 349.8 & 0 &  & \textbf{68.3} \\ 
  R\_300\_27209\_10\_75 & 290.0 & 0 &  & 95.5 & 108.4 & 0 &  & 97.0 & 122.8 & 0 &  & 98.2 & 551.4 & 0 &  & 90.1 & 439.6 & 0 &  & \textbf{78.2} \\ \hline
  R\_400\_2793\_10\_25 & 187.6 & 0 &  & 94.9 & 1996.6 & 0 &  & 23.0 & 2035.8 & 0 &  & 23.0 & 2142.0 & 0 &  & \textbf{18.9} & 2130.6 & 0 &  & 19.6 \\ 
  R\_400\_2793\_10\_50 & 842.0 & 0 &  & 89.9 & 3640.0 & 0 &  & 29.8 & 3734.2 & 0 &  & 29.3 & 4113.0 & 0 &  & \textbf{22.0} & 3924.8 & 0 &  & 29.0 \\ 
  R\_400\_2793\_10\_75 & 560.4 & 0 &  & 94.5 & 5130.0 & 0 &  & 27.4 & 5219.0 & 0 &  & 27.8 & 5611.6 & 0 &  & \textbf{22.1} & 5271.2 & 0 &  & 27.3 \\ \hline
  R\_400\_12369\_10\_25 & 0.0 & 0 &  & 100.0 & 493.2 & 0 &  & 72.7 & 699.2 & 0 &  & 74.0 & 700.0 & 0 &  & 68.5 & 696.0 & 0 &  & \textbf{65.1} \\ 
  R\_400\_12369\_10\_50 & 218.6 & 0 &  & 95.5 & 654.4 & 0 &  & 77.9 & 1262.0 & 0 &  & 69.5 & 1243.2 & 0 &  & \textbf{59.8} & 1230.6 & 0 &  & 59.9 \\ 
  R\_400\_12369\_10\_75 & 310.2 & 0 &  & 96.4 & 888.2 & 0 &  & 80.0 & 1819.6 & 0 &  & 72.1 & 1832.6 & 0 &  & 64.8 & 1805.6 & 0 &  & \textbf{62.7} \\ \hline
  R\_400\_48279\_10\_25 & 83.8 & 0 &  & 97.5 & 16.4 & 0 &  & 99.1 & 0.0 & 0 &  & 100.0 & 0.0 & 0 &  & 100.0 & 195.8 & 0 &  & \textbf{92.7} \\ 
  R\_400\_48279\_10\_50 & 116.6 & 0 &  & 97.6 & 79.2 & 0 &  & 96.9 & 0.0 & 0 &  & 100.0 & 0.0 & 0 &  & 100.0 & 381.8 & 0 &  & \textbf{90.0} \\ 
  R\_400\_48279\_10\_75 & 271.0 & 0 &  & 97.4 & 28.0 & 0 &  & 99.4 & 0.0 & 0 &  & 100.0 & 0.0 & 0 &  & 100.0 & 599.6 & 0 &  & \textbf{92.5} \\ \hline
  R\_500\_4241\_10\_25 & 0.0 & 0 &  & 100.0 & 2228.0 & 0 &  & \textbf{28.2} & 2129.6 & 0 &  & 34.7 & 2181.2 & 0 &  & 31.5 & 2300.0 & 0 &  & 28.8 \\ 
  R\_500\_4241\_10\_50 & 0.0 & 0 &  & 100.0 & 3656.2 & 0 &  & \textbf{30.7} & 3526.8 & 0 &  & 36.4 & 3617.2 & 0 &  & 33.1 & 3679.4 & 0 &  & 34.0 \\ 
  R\_500\_4241\_10\_75 & 0.0 & 0 &  & 100.0 & 5426.6 & 0 &  & 33.7 & 5403.8 & 0 &  & 37.5 & 5466.4 & 0 &  & 34.7 & 5658.2 & 0 &  & \textbf{33.4} \\ \hline
  R\_500\_19211\_10\_25 & 0.0 & 0 &  & 100.0 & 119.8 & 0 &  & 94.8 & 0.0 & 0 &  & 100.0 & 731.0 & 0 &  & 78.3 & 730.6 & 0 &  & \textbf{76.0} \\ 
  R\_500\_19211\_10\_50 & 0.0 & 0 &  & 100.0 & 413.2 & 0 &  & 87.5 & 258.6 & 0 &  & 94.5 & 1280.8 & 0 &  & 72.4 & 1264.6 & 0 &  & \textbf{70.0} \\ 
  R\_500\_19211\_10\_75 & 0.0 & 0 &  & 100.0 & 301.8 & 0 &  & 95.0 & 0.0 & 0 &  & 100.0 & 1975.2 & 0 &  & 76.5 & 1968.0 & 0 &  & \textbf{73.7} \\ \hline
  R\_500\_75349\_10\_25 & 0.0 & 0 &  & 100.0 & 51.2 & 0 &  & \textbf{98.3} & 0.0 & 0 &  & 100.0 & 0.0 & 0 &  & 100.0 & 0.0 & 0 &  & 100.0 \\ 
  R\_500\_75349\_10\_50 & 0.0 & 0 &  & 100.0 & 21.4 & 0 &  & \textbf{99.4} & 0.0 & 0 &  & 100.0 & 0.0 & 0 &  & 100.0 & 0.0 & 0 &  & 100.0 \\ 
  R\_500\_75349\_10\_75 & 0.0 & 0 &  & 100.0 & 30.4 & 0 &  & \textbf{99.6} & 0.0 & 0 &  & 100.0 & 0.0 & 0 &  & 100.0 & 0.0 & 0 &  & 100.0 \\ 
   \hline
     Average & 442.9 &  &  & 81.1 & 1324.6 &  & 418.7 & 60.1 & 1377.1 &  & 1648.9 & 57.5 & 1505.5 &  & 1287.5 & 55.5 & 1518.3 &  & 819.6 & 52.7 \\ 
  Total &  & 0 &  &  &  & 45 &  &  &  & 30 &  &  &  & 46 &  &  &  & 45 &  &  \\ 
   \hline
\end{tabular}
\end{table}


%\end{landscape}



%\begin{landscape}



\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations with warm start for the large square grid instances.}\label{tab:gridlargeinitsol}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
G\_10\_10\_10\_25 & 1504.0 & 5 & 71.2 &  & 1504.0 & 5 & \textbf{3.1} &  & 1504.0 & 5 & 3.6 &  & 1504.0 & 5 & 33.8 &  & 1504.0 & 5 & 5.6 &  \\ 
  G\_10\_10\_10\_50 & 2722.0 & 5 & 5.1 &  & 2722.0 & 5 & \textbf{1.4} &  & 2722.0 & 5 & 6.1 &  & 2722.0 & 5 & 8.1 &  & 2722.0 & 5 & 10.9 &  \\ 
  G\_10\_10\_10\_75 & 4307.6 & 5 & 6.2 &  & 4307.6 & 5 & \textbf{1.8} &  & 4307.6 & 5 & 5.4 &  & 4307.6 & 5 & 13.5 &  & 4307.6 & 5 & 37.5 &  \\ \hline
  G\_14\_14\_10\_25 & 2994.8 & 0 &  & 3.8 & 2996.2 & 5 & 1009.5 &  & 2996.2 & 5 & \textbf{32.2} &  & 2996.2 & 3 & 1058.0 & 0.1 & 2996.2 & 4 & 95.0 & 0.1 \\ 
  G\_14\_14\_10\_50 & 5489.0 & 0 &  & 1.9 & 5489.0 & 5 & 551.5 &  & 5489.0 & 5 & \textbf{152.5} &  & 5489.0 & 5 & 408.5 &  & 5489.0 & 1 & 2001.1 & 0.3 \\ 
  G\_14\_14\_10\_75 & 8806.4 & 0 &  & 2.9 & 8808.0 & 1 & 75.8 & 0.2 & 8808.2 & \textbf{5} & 64.6 &  & 8808.2 & 3 & 484.9 & 0.1 & 8805.4 & 2 & 94.5 & 0.3 \\ \hline
  G\_17\_17\_10\_25 & 4425.6 & 0 &  & 5.0 & 4426.6 & 0 &  & 0.2 & 4427.6 & \textbf{4} & 237.5 & 0.0 & 4427.6 & 1 & 2975.9 & 0.1 & 4423.0 & 1 & 233.9 & 0.4 \\ 
  G\_17\_17\_10\_50 & 8182.8 & 0 &  & 3.3 & 8185.6 & \textbf{5} & 775.9 &  & 8185.6 & 4 & 688.1 & 0.1 & 8185.6 & \textbf{5} & 1336.3 &  & 8181.6 & 1 & 847.3 & 0.3 \\ 
  G\_17\_17\_10\_75 & 13146.2 & 0 &  & 4.0 & 13155.2 & 1 & 3575.4 & 0.4 & 13155.2 & \textbf{5} & 828.0 &  & 13155.2 & 1 & 651.8 & 0.1 & 13142.6 & 0 &  & 0.3 \\ \hline
  G\_20\_20\_10\_25 & 6165.6 & 0 &  & 5.9 & 6171.4 & 0 &  & 0.3 & 6174.2 & \textbf{3} & 1837.5 & 0.0 & 6174.4 & 0 &  & 0.1 & 6160.8 & 0 &  & 0.4 \\ 
  G\_20\_20\_10\_50 & 11333.2 & 0 &  & 4.1 & 11344.4 & 0 &  & 0.3 & 11344.8 & \textbf{1} & 2840.8 & 0.1 & 11345.6 & 0 &  & 0.1 & 11332.6 & 0 &  & 0.5 \\ 
  G\_20\_20\_10\_75 & 18387.2 & 0 &  & 4.6 & 18402.2 & 0 &  & 0.5 & 18408.8 & \textbf{1} & 2554.7 & 0.0 & 18408.6 & 0 &  & 0.1 & 18379.2 & 0 &  & 0.4 \\ \hline
  G\_23\_23\_10\_25 & 8162.8 & 0 &  & 6.1 & 8169.6 & 0 &  & 0.3 & 8176.2 & \textbf{1} & 473.5 & 0.1 & 8172.8 & 0 &  & 0.2 & 8162.4 & 0 &  & 0.3 \\ 
  G\_23\_23\_10\_50 & 15174.4 & 0 &  & 4.4 & 15195.4 & 0 &  & 0.4 & 15197.4 & 0 &  & \textbf{0.1} & 15196.8 & 0 &  & 0.2 & 15161.0 & 0 &  & 0.6 \\ 
  G\_23\_23\_10\_75 & 24453.8 & 0 &  & 5.0 & 24491.6 & 0 &  & 0.5 & 24498.8 & 0 &  & \textbf{0.1} & 24504.6 & 0 &  & \textbf{0.1} & 24448.2 & 0 &  & 0.5 \\ \hline
  Average & 9017.0 &  & 27.5 & 4.2 & 9024.6 &  & 749.3 & 0.3 & 9026.4 &  & 748.1 & {0.1} & 9026.5 &  & 774.5 & {0.1} & 9014.4 &  & 415.7 & 0.4 \\ 
  Total &  & 15 &  &  &  & 32 &  &  &  & 49 &  &  &  & 33 &  &  &  & 24 &  &  \\ 
   \hline
\end{tabular}
\end{table}



\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations with warm start for the large nonsquare grid instances.}\label{tab:gridnqlargeinitsol}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
GNQ\_13\_7\_10\_25 & 1347.8 & 5 & 15.6 &  & 1347.8 & 5 & \textbf{1.8} &  & 1347.8 & 5 & 4.7 &  & 1347.8 & 5 & 23.4 &  & 1347.8 & 5 & 250.7 &  \\ 
  GNQ\_13\_7\_10\_50 & 2456.6 & 5 & 2.3 &  & 2456.6 & 5 & 1.3 &  & 2456.6 & 5 & \textbf{1.2} &  & 2456.6 & 5 & 1.9 &  & 2456.6 & 5 & 8.1 &  \\ 
  GNQ\_13\_7\_10\_75 & 3876.6 & 5 & 3.6 &  & 3876.6 & 5 & \textbf{1.5} &  & 3876.6 & 5 & 2.7 &  & 3876.6 & 5 & 11.3 &  & 3876.6 & 5 & 7.1 &  \\ \hline
  GNQ\_18\_11\_10\_25 & 3004.4 & 0 &  & 3.4 & 3005.0 & 4 & 227.2 & 0.2 & 3005.0 & \textbf{5} & 202.3 &  & 3005.0 & 4 & 1253.5 & 0.2 & 3004.0 & 1 & 77.7 & 0.2 \\ 
  GNQ\_18\_11\_10\_50 & 5509.8 & 0 &  & 2.2 & 5510.2 & 5 & \textbf{150.2} &  & 5510.2 & 5 & 162.0 &  & 5510.2 & 5 & 411.4 &  & 5509.4 & 3 & 120.2 & 0.4 \\ 
  GNQ\_18\_11\_10\_75 & 8827.6 & 0 &  & 2.6 & 8829.2 & 3 & 544.0 & 0.4 & 8829.6 & \textbf{5} & 148.7 &  & 8829.6 & 3 & 1237.7 & 0.1 & 8828.6 & 2 & 939.8 & 0.2 \\ \hline
  GNQ\_23\_13\_10\_25 & 4605.2 & 0 &  & 5.4 & 4608.2 & 0 &  & 0.2 & 4609.2 & \textbf{5} & 738.5 &  & 4609.2 & 0 &  & 0.1 & 4605.2 & 1 & 1515.2 & 0.2 \\ 
  GNQ\_23\_13\_10\_50 & 8446.2 & 0 &  & 3.5 & 8453.0 & 2 & 1358.1 & 0.3 & 8455.2 & \textbf{4} & 905.8 & 0.1 & 8455.2 & 4 & 1818.8 & 0.1 & 8443.2 & 0 &  & 0.5 \\ 
  GNQ\_23\_13\_10\_75 & 13587.0 & 0 &  & 4.1 & 13596.8 & 0 &  & 0.3 & 13599.4 & \textbf{4} & 1194.7 & 0.1 & 13599.4 & 1 & 1579.1 & 0.1 & 13581.6 & 0 &  & 0.3 \\ \hline
  GNQ\_26\_15\_10\_25 & 5997.8 & 0 &  & 5.8 & 6004.4 & 0 &  & 0.2 & 6005.8 & \textbf{5} & 1690.5 &  & 6005.6 & 0 &  & 0.1 & 5996.8 & 0 &  & 0.3 \\ 
  GNQ\_26\_15\_10\_50 & 11092.0 & 0 &  & 3.6 & 11098.8 & 1 & 532.8 & 0.3 & 11098.6 & \textbf{2} & 1995.1 & 0.1 & 11099.0 & 1 & 1533.7 & 0.1 & 11091.0 & 1 & 1603.0 & 0.4 \\ 
  GNQ\_26\_15\_10\_75 & 17887.0 & 0 &  & 4.6 & 17899.2 & 0 &  & 0.4 & 17906.0 & \textbf{4} & 973.2 & 0.0 & 17905.4 & 0 &  & 0.1 & 17875.6 & 0 &  & 0.3 \\ \hline
  GNQ\_29\_17\_10\_25 & 7621.6 & 0 &  & 6.2 & 7626.8 & 0 &  & 0.2 & 7627.6 & \textbf{3} & 2371.0 & 0.1 & 7626.8 & 0 &  & 0.1 & 7618.8 & 0 &  & 0.2 \\ 
  GNQ\_29\_17\_10\_50 & 14048.8 & 0 &  & 4.4 & 14061.0 & 0 &  & 0.4 & 14064.8 & 0 &  & \textbf{0.1} & 14064.6 & 0 &  & 0.2 & 14038.2 & 0 &  & 0.7 \\ 
  GNQ\_29\_17\_10\_75 & 22743.8 & 0 &  & 4.7 & 22767.0 & 0 &  & 0.4 & 22767.0 & 0 &  & \textbf{0.1} & 22767.0 & 0 &  & 0.2 & 22733.8 & 0 &  & 0.4 \\ \hline
  Average & 8736.8 &  & 7.2 & 4.2 & 8742.7 &  & 352.1 & 0.3 & 8744.0 &  & 799.3 & \textbf{0.1} & 8743.9 &  & 874.5 & \textbf{0.1} & 8733.8 &  & 565.2 & 0.3 \\ 
  Total &  & 15 &  &  &  & 30 &  &  &  & 57 &  &  &  & 33 &  &  &  & 23 &  &  \\ 
   \hline
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations with warm start for the large hypercube instances.}\label{tab:ipercubelargeinitsol}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
I\_7\_10\_25 & 1037.4 & 0 &  & 13.2 & 1037.4 & 0 &  & 1.4 & 1037.4 & 0 &  & 1.9 & 1037.4 & \textbf{1} & 2489.6 & 1.4 & 1037.4 & 0 &  & 2.8 \\ 
  I\_7\_10\_50 & 1935.6 & 0 &  & 5.8 & 1935.6 & 5 & 222.8 &  & 1935.6 & 5 & 317.4 &  & 1935.6 & 5 & \textbf{135.8} &  & 1935.6 & 4 & 63.8 & 1.1 \\ 
  I\_7\_10\_75 & 2533.6 & 0 &  & 3.8 & 2533.6 & 5 & 26.9 &  & 2533.6 & 5 & 16.6 &  & 2533.6 & 5 & \textbf{7.1} &  & 2533.6 & 5 & 42.1 &  \\ \hline
  I\_8\_10\_25 & 2047.4 & 0 &  & 18.5 & 2044.8 & 0 &  & 3.6 & 2058.2 & 0 &  & 3.4 & 2065.4 & 0 &  & \textbf{2.3} & 2058.8 & 0 &  & 3.1 \\ 
  I\_8\_10\_50 & 3714.0 & 0 &  & 13.6 & 3714.0 & 0 &  & 3.1 & 3714.0 & 0 &  & 2.4 & 3714.0 & 0 &  & \textbf{1.6} & 3714.0 & 0 &  & 2.2 \\ 
  I\_8\_10\_75 & 4948.4 & 0 &  & 10.2 & 4948.4 & 0 &  & 1.5 & 4948.4 & 1 & 654.4 & 0.6 & 4948.4 & \textbf{4} & 451.4 & 0.5 & 4948.4 & \textbf{4} & 1398.5 & 1.1 \\ \hline
  I\_9\_10\_25 & 3944.8 & 0 &  & 23.1 & 3944.8 & 0 &  & 5.7 & 3944.8 & 0 &  & 5.7 & 3952.6 & 0 &  & \textbf{5.3} & 3944.8 & 0 &  & 5.6 \\ 
  I\_9\_10\_50 & 7317.0 & 0 &  & 17.8 & 7317.0 & 0 &  & 5.0 & 7317.0 & 0 &  & 4.3 & 7324.4 & 0 &  & \textbf{3.9} & 7317.0 & 0 &  & 4.0 \\ 
  I\_9\_10\_75 & 9341.0 & 0 &  & 15.3 & 9341.0 & 0 &  & 3.9 & 9342.3 & 0 &  & 2.8 & 9343.7 & 0 &  & \textbf{2.4} & 9342.3 & 0 &  & \textbf{2.4} \\ \hline
  Average & 4091.0 &  &  & 13.5 & 4090.7 &  & 124.9 & 3.5 & 4092.4 &  & 329.5 & 3.0 & 4095.0 &  & 771.0 & {2.5} & 4092.4 &  & 501.5 & 2.8 \\ 
  Total &  & 0 &  &  &  & 10 &  &  &  & 11 &  &  &  & 15 &  &  &  & 13 &  &  \\ 
   \hline
\end{tabular}
\end{table}

% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Thu Oct  8 13:47:11 2020
\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations with warm start for the large toroidal instances.}\label{tab:torolargeinitsol}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
T\_10\_10\_10\_25 & 946.2 & 0 &  & 2.9 & 946.2 & 5 & 19.4 &  & 946.2 & 5 & 8.5 &  & 946.2 & 5 & 34.8 &  & 946.2 & 5 & \textbf{7.9} &  \\ 
  T\_10\_10\_10\_50 & 1350.4 & 5 & 1040.0 &  & 1350.4 & 5 & 4.2 &  & 1350.4 & 5 & \textbf{3.4} &  & 1350.4 & 5 & 15.3 &  & 1350.4 & 5 & 100.4 &  \\ 
  T\_10\_10\_10\_75 & 1778.0 & 5 & 69.5 &  & 1778.0 & 5 & 2.1 &  & 1778.0 & 5 & \textbf{1.4} &  & 1778.0 & 5 & 1.8 &  & 1778.0 & 4 & 3.9 & 0.6 \\ \hline
  T\_14\_14\_10\_25 & 1840.0 & 0 &  & 4.9 & 1840.0 & 1 & 11.1 & 0.5 & 1840.6 & 5 & \textbf{407.9} &  & 1840.6 & 5 & 676.2 &  & 1840.6 & 5 & 453.7 &  \\ 
  T\_14\_14\_10\_50 & 2801.6 & 0 &  & 2.1 & 2801.6 & 3 & 110.6 & 0.3 & 2801.6 & \textbf{5} & 50.5 &  & 2801.6 & \textbf{5} & 94.5 &  & 2801.6 & 4 & 555.9 & 0.3 \\ 
  T\_14\_14\_10\_75 & 3728.2 & 1 & 1194.3 & 1.1 & 3728.2 & 5 & 64.0 &  & 3728.2 & 5 & \textbf{53.4} &  & 3728.2 & 5 & 55.2 &  & 3728.2 & 0 &  & 0.5 \\ \hline
  T\_17\_17\_10\_25 & 2738.2 & 0 &  & 5.5 & 2738.2 & 0 &  & 0.6 & 2740.0 & \textbf{2} & 942.0 & 0.1 & 2740.0 & 1 & 287.9 & 0.1 & 2738.4 & \textbf{2} & 541.6 & 0.5 \\ 
  T\_17\_17\_10\_50 & 4110.8 & 0 &  & 2.9 & 4110.8 & 0 &  & 0.4 & 4112.4 & \textbf{5} & 500.2 &  & 4112.4 & \textbf{5} & 762.7 &  & 4110.8 & 1 & 1285.2 & 0.6 \\ 
  T\_17\_17\_10\_75 & 5476.8 & 0 &  & 1.8 & 5477.0 & 2 & 1424.9 & 0.3 & 5477.8 & \textbf{5} & 723.2 &  & 5477.8 & \textbf{5} & 403.8 &  & 5476.8 & 0 &  & 0.8 \\ \hline
  T\_20\_20\_10\_25 & 3793.0 & 0 &  & 6.2 & 3793.0 & 0 &  & 0.8 & 3801.0 & \textbf{1} & 3461.2 & 0.2 & 3800.0 & 0 &  & 0.2 & 3794.6 & 0 &  & 0.6 \\ 
  T\_20\_20\_10\_50 & 5619.2 & 0 &  & 3.2 & 5620.0 & 0 &  & 0.5 & 5622.2 & \textbf{4} & 2302.7 & 0.1 & 5622.2 & 2 & 2144.7 & 0.1 & 5619.2 & 0 &  & 0.6 \\ 
  T\_20\_20\_10\_75 & 7381.2 & 0 &  & 2.0 & 7382.8 & 0 &  & 0.3 & 7383.8 & \textbf{5} & 1447.6 &  & 7383.8 & 4 & 886.3 & 0.1 & 7381.2 & 0 &  & 0.6 \\ \hline
  T\_23\_23\_10\_25 & 4996.0 & 0 &  & 6.5 & 4996.0 & 0 &  & 0.9 & 5007.8 & 0 &  & 0.3 & 5004.5 & 0 &  & 0.4 & 4999.2 & 0 &  & 0.6 \\ 
  T\_23\_23\_10\_50 & 7545.2 & 0 &  & 3.2 & 7547.6 & 0 &  & 0.5 & 7552.6 & \textbf{1} & 2526.1 & 0.1 & 7552.0 & \textbf{1} & 3105.0 & 0.1 & 7545.2 & 0 &  & 0.8 \\ 
  T\_23\_23\_10\_75 & 10112.2 & 0 &  & 2.2 & 10113.8 & 0 &  & 0.4 & 10116.2 & 1 & 2847.3 & 0.1 & 10116.2 & \textbf{2} & 2359.1 & 0.1 & 10112.0 & 0 &  & 0.8 \\ \hline
  Average & 4281.1 &  & 767.9 & 3.4 & 4281.6 &  & 233.8 & 0.5 & 4283.9 &  & 1091.1 & 0.1 & 4283.6 &  & 832.9 & 0.2 & 4281.5 &  & 421.2 & 0.6 \\ 
  Total &  & 11 &  &  &  & 26 &  &  &  & 54 &  &  &  & 50 &  &  &  & 26 &  &  \\ 
   \hline
\end{tabular}
\end{table}




\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations with warm start for the large random instances.}\label{tab:randlargeinitsol}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
  R\_100\_247\_10\_25 & 1004.6 & 0 &  & 6.7 & 1004.6 & 5 & 11.7 &  & 1004.6 & 5 & 6.5 &  & 1004.6 & 5 & \textbf{5.1} &  & 1004.6 & 5 & 5.4 &  \\ 
  R\_100\_247\_10\_50 & 1696.4 & 0 &  & 6.0 & 1696.4 & 5 & 56.0 &  & 1696.4 & 5 & \textbf{7.0} &  & 1696.4 & 5 & \textbf{7.0} &  & 1696.4 & 5 & 8.9 &  \\ 
  R\_100\_247\_10\_75 & 2449.2 & 0 &  & 5.5 & 2449.2 & 5 & 52.3 &  & 2449.2 & 5 & 6.4 &  & 2449.2 & 5 & \textbf{4.5} &  & 2449.2 & 5 & 8.3 &  \\ \hline
  R\_100\_841\_10\_25 & 492.0 & 0 &  & 28.3 & 492.0 & 5 & \textbf{117.2} &  & 492.0 & 5 & 1928.0 &  & 492.0 & 5 & 788.4 &  & 492.0 & 5 & 1008.9 &  \\ 
  R\_100\_841\_10\_50 & 949.8 & 0 &  & 29.8 & 949.8 & 5 & \textbf{210.2} &  & 949.8 & 5 & 2521.2 &  & 949.8 & 5 & 961.7 &  & 949.8 & 5 & 1022.5 &  \\ 
  R\_100\_841\_10\_75 & 1350.8 & 0 &  & 28.9 & 1350.8 & 5 & \textbf{181.2} &  & 1350.8 & 5 & 1877.5 &  & 1350.8 & 5 & 759.5 &  & 1350.8 & 5 & 826.8 &  \\ \hline
  R\_100\_3069\_10\_25 & 169.6 & 0 &  & 66.4 & 169.6 & 5 & \textbf{827.4} &  & 169.6 & 0 &  & 34.6 & 169.6 & 5 & 2589.2 &  & 169.6 & 5 & 1004.4 &  \\ 
  R\_100\_3069\_10\_50 & 326.4 & 0 &  & 64.7 & 326.8 & 5 & 683.3 &  & 326.4 & 1 & 3190.4 & 27.7 & 326.4 & 5 & 1879.3 &  & 326.4 & 5 & \textbf{557.4} &  \\ 
  R\_100\_3069\_10\_75 & 489.8 & 0 &  & 63.7 & 489.8 & 5 & 602.9 &  & 489.8 & 1 & 2817.0 & 23.6 & 489.8 & 5 & 1738.9 &  & 489.8 & 5 & \textbf{453.6} &  \\ \hline
  R\_200\_796\_10\_25 & 1687.6 & 0 &  & 23.9 & 1687.6 & 0 &  & 2.9 & 1687.6 & 0 &  & 4.2 & 1687.8 & 0 &  & \textbf{2.8} & 1689.4 & 0 &  & 3.2 \\ 
  R\_200\_796\_10\_50 & 2828.6 & 0 &  & 22.8 & 2828.6 & 0 &  & 2.9 & 2828.6 & 0 &  & 4.0 & 2829.4 & 0 &  & \textbf{2.2} & 2828.8 & 0 &  & 2.7 \\ 
  R\_200\_796\_10\_75 & 3768.2 & 0 &  & 21.4 & 3768.2 & 0 &  & 2.7 & 3768.2 & 0 &  & 3.3 & 3768.2 & 1 & 2751.6 & \textbf{1.7} & 3768.2 & 0 &  & 2.4 \\ \hline
  R\_200\_3184\_10\_25 & 678.0 & 0 &  & 55.9 & 678.0 & 0 &  & \textbf{26.7} & 678.0 & 0 &  & 33.2 & 678.0 & 0 &  & 27.5 & 678.0 & 0 &  & 30.0 \\ 
  R\_200\_3184\_10\_50 & 1233.6 & 0 &  & 56.4 & 1233.6 & 0 &  & 27.6 & 1233.6 & 0 &  & 34.1 & 1233.6 & 0 &  & \textbf{27.3} & 1233.6 & 0 &  & 30.4 \\ 
  R\_200\_3184\_10\_75 & 1773.8 & 0 &  & 55.4 & 1773.8 & 0 &  & \textbf{25.7} & 1773.8 & 0 &  & 32.8 & 1773.8 & 0 &  & 26.2 & 1773.8 & 0 &  & 28.9 \\ \hline
  R\_200\_12139\_10\_25 & 210.2 & 0 &  & 83.3 & 210.2 & 0 &  & 74.1 & 210.2 & 0 &  & 82.9 & 210.2 & 0 &  & 78.3 & 210.2 & 0 &  & \textbf{54.7} \\ 
  R\_200\_12139\_10\_50 & 378.2 & 0 &  & 81.9 & 378.2 & 0 &  & 72.4 & 378.2 & 0 &  & 80.8 & 378.2 & 0 &  & 75.8 & 378.2 & 0 &  & \textbf{50.9} \\ 
  R\_200\_12139\_10\_75 & 540.2 & 0 &  & 80.9 & 540.2 & 0 &  & 70.6 & 540.2 & 0 &  & 81.5 & 540.2 & 0 &  & 74.6 & 540.2 & 0 &  & \textbf{48.6} \\ \hline
  R\_300\_1644\_10\_25 & 1984.8 & 0 &  & 30.4 & 1984.8 & 0 &  & \textbf{6.4} & 1984.8 & 0 &  & 8.5 & 1984.8 & 0 &  & 7.5 & 1984.8 & 0 &  & 7.3 \\ 
  R\_300\_1644\_10\_50 & 3574.2 & 0 &  & 34.1 & 3574.2 & 0 &  & \textbf{9.1} & 3574.2 & 0 &  & 11.2 & 3574.2 & 0 &  & 10.1 & 3574.2 & 0 &  & 10.0 \\ 
  R\_300\_1644\_10\_75 & 5291.4 & 0 &  & 33.5 & 5291.4 & 0 &  & \textbf{8.8} & 5291.4 & 0 &  & 10.8 & 5291.4 & 0 &  & 9.8 & 5291.4 & 0 &  & 10.0 \\ \hline
  R\_300\_7026\_10\_25 & 782.0 & 0 &  & 67.8 & 782.0 & 0 &  & \textbf{43.1} & 782.0 & 0 &  & 52.4 & 782.0 & 0 &  & 46.7 & 782.0 & 0 &  & 46.6 \\ 
  R\_300\_7026\_10\_50 & 1493.0 & 0 &  & 67.8 & 1493.0 & 0 &  & \textbf{42.2} & 1493.0 & 0 &  & 51.6 & 1493.0 & 0 &  & 46.8 & 1493.0 & 0 &  & 46.9 \\ 
  R\_300\_7026\_10\_75 & 2099.8 & 0 &  & 67.2 & 2099.8 & 0 &  & \textbf{41.9} & 2099.8 & 0 &  & 50.8 & 2099.8 & 0 &  & 46.4 & 2099.8 & 0 &  & 46.7 \\ \hline
  R\_300\_27209\_10\_25 & 229.2 & 0 &  & 88.8 & 229.2 & 0 &  & 81.6 & 229.2 & 0 &  & 94.2 & 229.2 & 0 &  & 88.5 & 229.2 & 0 &  & \textbf{67.4} \\ 
  R\_300\_27209\_10\_50 & 415.0 & 0 &  & 86.7 & 415.0 & 0 &  & 77.4 & 415.0 & 0 &  & 90.7 & 415.0 & 0 &  & 86.3 & 415.0 & 0 &  & \textbf{61.4} \\ 
  R\_300\_27209\_10\_75 & 691.0 & 0 &  & 88.1 & 691.0 & 0 &  & 79.4 & 691.0 & 0 &  & 92.7 & 691.0 & 0 &  & 87.6 & 691.0 & 0 &  & \textbf{64.2} \\ \hline
  R\_400\_2793\_10\_25 & 2270.0 & 0 &  & 39.8 & 2270.0 & 0 &  & \textbf{12.0} & 2270.0 & 0 &  & 14.4 & 2270.0 & 0 &  & 14.2 & 2270.0 & 0 &  & 13.8 \\ 
  R\_400\_2793\_10\_50 & 4365.4 & 0 &  & 42.6 & 4365.4 & 0 &  & \textbf{15.3} & 4365.4 & 0 &  & 17.6 & 4365.4 & 0 &  & 17.3 & 4365.4 & 0 &  & 17.0 \\ 
  R\_400\_2793\_10\_75 & 6020.2 & 0 &  & 42.2 & 6020.2 & 0 &  & \textbf{14.7} & 6020.2 & 0 &  & 16.7 & 6020.2 & 0 &  & 16.5 & 6020.2 & 0 &  & 16.3 \\ \hline
  R\_400\_12369\_10\_25 & 860.4 & 0 &  & 76.2 & 860.4 & 0 &  & \textbf{52.8} & 860.4 & 0 &  & 68.1 & 860.4 & 0 &  & 59.4 & 860.4 & 0 &  & 56.4 \\ 
  R\_400\_12369\_10\_50 & 1495.4 & 0 &  & 72.3 & 1495.4 & 0 &  & \textbf{47.1} & 1495.4 & 0 &  & 64.1 & 1495.4 & 0 &  & 54.1 & 1495.4 & 0 &  & 51.3 \\ 
  R\_400\_12369\_10\_75 & 2195.8 & 0 &  & 74.4 & 2195.8 & 0 &  & \textbf{50.5} & 2195.8 & 0 &  & 66.5 & 2195.8 & 0 &  & 60.0 & 2195.8 & 0 &  & 53.9 \\ \hline
  R\_400\_48279\_10\_25 & 245.6 & 0 &  & 92.3 & 245.6 & 0 &  & \textbf{85.0} & 245.6 & 0 &  & 95.4 & 245.6 & 0 &  & 95.4 & 245.6 & 0 &  & 90.8 \\ 
  R\_400\_48279\_10\_50 & 445.0 & 0 &  & 90.4 & 445.0 & 0 &  & \textbf{80.1} & 445.0 & 0 &  & 94.1 & 445.0 & 0 &  & 94.1 & 445.0 & 0 &  & 88.3 \\ 
  R\_400\_48279\_10\_75 & 766.6 & 0 &  & 92.1 & 766.6 & 0 &  & \textbf{83.3} & 766.6 & 0 &  & 95.2 & 766.6 & 0 &  & 95.2 & 766.6 & 0 &  & 90.4 \\ \hline
  R\_500\_4241\_10\_25 & 2561.8 & 0 &  & 49.8 & 2561.8 & 0 &  & \textbf{17.3} & 2561.8 & 0 &  & 21.4 & 2561.8 & 0 &  & 19.6 & 2561.8 & 0 &  & 19.3 \\ 
  R\_500\_4241\_10\_50 & 4277.2 & 0 &  & 50.0 & 4277.2 & 0 &  & \textbf{19.3} & 4277.2 & 0 &  & 23.2 & 4277.2 & 0 &  & 21.2 & 4277.2 & 0 &  & 21.1 \\ 
  R\_500\_4241\_10\_75 & 6613.8 & 0 &  & 50.1 & 6613.8 & 0 &  & \textbf{19.3} & 6613.8 & 0 &  & 23.7 & 6613.8 & 0 &  & 21.3 & 6613.8 & 0 &  & 21.2 \\ \hline
  R\_500\_19211\_10\_25 & 919.4 & 0 &  & 82.4 & 919.4 & 0 &  & \textbf{60.3} & 919.4 & 0 &  & 86.2 & 919.4 & 0 &  & 72.7 & 919.4 & 0 &  & 69.6 \\ 
  R\_500\_19211\_10\_50 & 1540.0 & 0 &  & 78.0 & 1540.0 & 0 &  & \textbf{53.2} & 1540.0 & 0 &  & 70.7 & 1540.0 & 0 &  & 66.2 & 1540.0 & 0 &  & 62.8 \\ 
  R\_500\_19211\_10\_75 & 2381.4 & 0 &  & 81.7 & 2381.4 & 0 &  & \textbf{58.9} & 2381.4 & 0 &  & 82.7 & 2381.4 & 0 &  & 71.6 & 2381.4 & 0 &  & 68.4 \\ \hline
  R\_500\_75349\_10\_25 & 0.0 &  &  &  & 259.8 & 0 &  & \textbf{89.4} & 259.8 & 0 &  & 96.1 & 259.8 & 0 &  & 96.1 & 259.8 & 0 &  & 96.1 \\ 
  R\_500\_75349\_10\_50 & 0.0 &  &  &  & 450.8 & 0 &  & \textbf{85.7} & 450.8 & 0 &  & 95.1 & 450.8 & 0 &  & 95.1 & 450.8 & 0 &  & 95.1 \\ 
  R\_500\_75349\_10\_75 & 0.0 &  &  &  & 760.4 & 0 &  & \textbf{88.7} & 760.4 & 0 &  & 95.5 & 760.4 & 0 &  & 95.5 & 760.4 & 0 &  & 95.5 \\ \hline
  Average & 1678.8 &  &  & 56.2 & 1711.5 &  & 304.7 & 45.2 & 1711.5 &  & 1544.3 & 52.1 & 1711.5 &  & 1148.5 & 50.3 & 1711.5 &  & 544.0 & 45.5 \\ 
  Total &  & 0 &  &  &  & 45 &  &  &  & 32 &  &  &  & 46 &  &  &  & 45 &  &  \\ 
 
   \hline
\end{tabular}
\end{table}





\end{landscape}

The plots in Figure~\ref{fig:comparison-large-instances}
compare the average fraction in percent over all individual large instances solved to optimality within the time limit of 3600 seconds in each class for each formulation, (a) using the standalone formulations and (b) running with feasible warm starts generated by the matheuristic MILS$^+$-$mtz$ described in Section 3.6 of~\citeA{MelQueRib21}.
The plots show that FLOW performs the best for 
%all but the hypercube \rafaelC{and random classes}. 
three out of the five classes (square grid, non-square grid, and toroidal).
They also illustrate, once again, that formulation DCUT is the mostly benefited by the warm starts.

\begin{figure}[H]
\begin{center}
    \begin{tabular}{cc}
    \includegraphics[width=0.5\textwidth]{optimal_Large_original.pdf} & \includegraphics[width=0.5\textwidth]{optimal_Large_initialsolution.pdf}\\
(a) Standalone formulations & (b) Running with warm starts
%  (a) Aggregated results for small instances  & (b) Aggregated results for small instances\\    running as standalone formulations & with warm starts
\end{tabular}
\end{center}
\caption{Average fraction in percent over all individual large instances solved to optimality in each class for each formulation, (a) first using the standalone formulations, and (b) then running with feasible warm starts generated by the matheuristic MILS$^+$-$mtz$. For each instance, the computation time considered in the averages is either the time to prove optimality (if less than the imposed time limit of 3600 seconds) or this imposed time limit.}\label{fig:comparison-large-instances}
\end{figure}


\subsection{Small instances when disabling solver's features}

In order to have an idea of the behavior of the formulations when used in MIP solvers with different \rafaelC{capabilities, Tables}~\ref{tab:gridinitsoldisable}-\ref{tab:randinitsoldisable} show the results for the small instances when turning off the solver's heuristics and built-in cutting planes and allowing just a single thread (i.e., no parallelism). These tables indicate that under this setting, only TCYC and MTZ were able to solve all the small instances to optimality. TCYC has shown to be the most effective approach for the small instances when we consider the average times, as it obtained the best overall averages for the majority of the graph classes.

%\celsoF{E não faz sentido testar ou pelo menos comentar sobre a desabilitação das features do solver nas instancias grandes?} \rafaelF{Esse tipo de coisa depende muito de revisor. Tem escola que desabilita tudo pra testar somente os métodos, tentando minimizar o efeito do solver. Tem escola que considera válido usar tudo o que está disponível no solver. Eu normalmente sigo mais a segunda. No intuito de pelo menos responder a algum questionamento sobre dependência do solver, foi que eu propus colocar pelo menos para as pequenas. Rodar tudo para as grandes vai ser muita coisa, e muita tabela. Talvez possamos somente fazer uma observação introduzindo que o objetivo não é fazer experimentos estensivos, e  concluindo que há um décrescimo na performance de todas as abordagens, mas comparativamente, não há muita diferença e, além disso, parecem estar mais a favor de TCYC. O que acha?}
















\begin{landscape}

% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Fri Oct 23 07:47:29 2020
\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations with warm start for the small square grid instances disabling the solver's preprocessing, cuts and heuristics.}\label{tab:gridinitsoldisable}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
G\_5\_5\_10\_25 & 352.4 & 5 & 1.2 &  & 352.4 & 5 & 0.9 &  & 352.4 & 5 & \textbf{0.0} &  & 352.4 & 5 & 0.1 &  & 352.4 & 5 & 1.4 &  \\ 
  G\_5\_5\_10\_50 & 636.8 & 5 & 1.2 &  & 636.8 & 5 & 0.9 &  & 636.8 & 5 & \textbf{0.0} &  & 636.8 & 5 & 0.1 &  & 636.8 & 5 & 1.4 &  \\ 
  G\_5\_5\_10\_75 & 934.2 & 5 & 1.2 &  & 934.2 & 5 & 0.9 &  & 934.2 & 5 & \textbf{0.0} &  & 934.2 & 5 & 0.1 &  & 934.2 & 5 & 1.6 &  \\ \hline
  G\_7\_7\_10\_25 & 712.4 & 5 & 1.3 &  & 712.4 & 5 & 0.9 &  & 712.4 & 5 & \textbf{0.3} &  & 712.4 & 5 & 1.3 &  & 712.4 & 5 & 1.8 &  \\ 
  G\_7\_7\_10\_50 & 1324.2 & 5 & 1.2 &  & 1324.2 & 5 & 0.9 &  & 1324.2 & 5 & \textbf{0.1} &  & 1324.2 & 5 & 0.4 &  & 1324.2 & 5 & 1.6 &  \\ 
  G\_7\_7\_10\_75 & 1998.6 & 5 & 1.3 &  & 1998.6 & 5 & 0.9 &  & 1998.6 & 5 & \textbf{0.2} &  & 1998.6 & 5 & 0.7 &  & 1998.6 & 5 & 1.7 &  \\ \hline
  G\_9\_9\_10\_25 & 1180.8 & 5 & 32.1 &  & 1180.8 & 5 & \textbf{1.9} &  & 1180.8 & 5 & 4.5 &  & 1180.8 & 5 & 23.6 &  & 1180.8 & 5 & 10.2 &  \\ 
  G\_9\_9\_10\_50 & 2192.2 & 5 & 3.0 &  & 2192.2 & 5 & \textbf{1.2} &  & 2192.2 & 5 & 4.1 &  & 2192.2 & 5 & 7.9 &  & 2192.2 & 5 & 25.4 &  \\ 
  G\_9\_9\_10\_75 & 3452.2 & 5 & 2.1 &  & 3452.2 & 5 & 1.1 &  & 3452.2 & 5 & \textbf{1.0} &  & 3452.2 & 5 & 4.5 &  & 3452.2 & 5 & 2.9 &  \\ \hline
  Average & 1420.4 &  & 5.0 &  & 1420.4 &  & 1.1 &  & 1420.4 &  & 1.1 &  & 1420.4 &  & 4.3 &  & 1420.4 &  & 5.3 &  \\ 
  Total &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  \\ 
   \hline
\end{tabular}
\end{table}

% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Fri Oct 23 07:48:00 2020
\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations with warm start for the small nonsquare grid instances disabling the solver's preprocessing, cuts and heuristics.}\label{tab:gridnqinitsoldisable}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
GNQ\_8\_3\_10\_25 & 319.2 & 5 & 1.2 &  & 319.2 & 5 & 0.9 &  & 319.2 & 5 & \textbf{0.0} &  & 319.2 & 5 & 0.1 &  & 319.2 & 5 & 1.6 &  \\ 
  GNQ\_8\_3\_10\_50 & 579.2 & 5 & 1.2 &  & 579.2 & 5 & 0.9 &  & 579.2 & 5 & \textbf{0.0} &  & 579.2 & 5 & \textbf{0.0} &  & 579.2 & 5 & 1.6 &  \\ 
  GNQ\_8\_3\_10\_75 & 838.0 & 5 & 1.2 &  & 838.0 & 5 & 0.9 &  & 838.0 & 5 & \textbf{0.0} &  & 838.0 & 5 & 0.0 &  & 838.0 & 5 & 1.4 &  \\ \hline
  GNQ\_9\_6\_10\_25 & 786.8 & 5 & 1.6 &  & 786.8 & 5 & 1.0 &  & 786.8 & 5 & \textbf{0.4} &  & 786.8 & 5 & 4.4 &  & 786.8 & 5 & 1.7 &  \\ 
  GNQ\_9\_6\_10\_50 & 1438.6 & 5 & 1.3 &  & 1438.6 & 5 & 1.0 &  & 1438.6 & 5 & \textbf{0.5} &  & 1438.6 & 5 & 1.8 &  & 1438.6 & 5 & 2.7 &  \\ 
  GNQ\_9\_6\_10\_75 & 2195.6 & 5 & 1.3 &  & 2195.6 & 5 & 1.0 &  & 2195.6 & 5 & \textbf{0.3} &  & 2195.6 & 5 & 1.1 &  & 2195.6 & 5 & 2.1 &  \\ \hline
  GNQ\_12\_6\_10\_25 & 1071.2 & 5 & 3.8 &  & 1071.2 & 5 & \textbf{1.3} &  & 1071.2 & 5 & 2.9 &  & 1071.2 & 5 & 17.3 &  & 1071.2 & 5 & 36.8 &  \\ 
  GNQ\_12\_6\_10\_50 & 1944.2 & 5 & 1.9 &  & 1944.2 & 5 & \textbf{1.1} &  & 1944.2 & 5 & 2.9 &  & 1944.2 & 5 & 8.0 &  & 1944.2 & 5 & 27.6 &  \\ 
  GNQ\_12\_6\_10\_75 & 3022.4 & 5 & 1.5 &  & 3022.4 & 5 & \textbf{1.0} &  & 3022.4 & 5 & 1.4 &  & 3022.4 & 5 & 4.4 &  & 3022.4 & 5 & 7.1 &  \\ \hline
  Average & 1355.0 &  & 1.7 &  & 1355.0 &  & 1.0 &  & 1355.0 &  & 0.9 &  & 1355.0 &  & 4.1 &  & 1355.0 &  & 9.2 &  \\ 
  Total &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  \\ 
   \hline
\end{tabular}
\end{table}



% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Fri Oct 23 07:48:23 2020
\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations with warm start for the small hypercube instances disabling the solver's preprocessing, cuts and heuristics.}\label{tab:ipercubeinitsoldisable}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
I\_4\_10\_25 & 147.0 & 5 & 1.2 &  & 147.0 & 5 & 0.9 &  & 147.0 & 5 & \textbf{0.0} &  & 147.0 & 5 & \textbf{0.0} &  & 147.0 & 5 & 1.5 &  \\ 
  I\_4\_10\_50 & 289.4 & 5 & 1.2 &  & 289.4 & 5 & 0.9 &  & 289.4 & 5 & \textbf{0.0} &  & 289.4 & 5 & \textbf{0.0} &  & 289.4 & 5 & 1.5 &  \\ 
  I\_4\_10\_75 & 344.0 & 5 & 1.2 &  & 344.0 & 5 & 0.9 &  & 344.0 & 5 & \textbf{0.0} &  & 344.0 & 5 & \textbf{0.0} &  & 344.0 & 5 & 1.5 &  \\ \hline
  I\_5\_10\_25 & 278.4 & 5 & 2.4 &  & 278.4 & 5 & \textbf{1.3} &  & 278.4 & 5 & 1.4 &  & 278.4 & 5 & 1.5 &  & 278.4 & 5 & 3.4 &  \\ 
  I\_5\_10\_50 & 545.0 & 5 & 1.4 &  & 545.0 & 5 & 1.0 &  & 545.0 & 5 & \textbf{0.2} &  & 545.0 & 5 & \textbf{0.2} &  & 545.0 & 5 & 1.6 &  \\ 
  I\_5\_10\_75 & 787.4 & 5 & 1.3 &  & 787.4 & 5 & 0.9 &  & 787.4 & 5 & \textbf{0.1} &  & 787.4 & 5 & \textbf{0.1} &  & 787.4 & 5 & 1.6 &  \\ \hline
  I\_6\_10\_25 & 527.2 & 0 &  & 4.9 & 527.2 & 5 & \textbf{67.2} &  & 527.2 & 5 & 177.3 &  & 527.2 & 5 & 88.9 &  & 527.2 & 2 & 870.8 & 2.4 \\ 
  I\_6\_10\_50 & 975.6 & 5 & 73.2 &  & 975.6 & 5 & \textbf{5.2} &  & 975.6 & 5 & 13.4 &  & 975.6 & 5 & 8.6 &  & 975.6 & 5 & 136.7 &  \\ 
  I\_6\_10\_75 & 1250.8 & 5 & 12.0 &  & 1250.8 & 5 & 1.4 &  & 1250.8 & 5 & 1.1 &  & 1250.8 & 5 & \textbf{1.0} &  & 1250.8 & 5 & 3.2 &  \\ \hline
  Average & 571.6 &  & 11.7 & 4.9 & 571.6 &  & 8.8 &  & 571.6 &  & 21.5 &  & 571.6 &  & 11.1 &  & 571.6 &  & 113.5 & 2.4 \\ 
  Total &  & 40 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 42 &  &  \\ 
   \hline
\end{tabular}
\end{table}



% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Fri Oct 23 07:48:55 2020
\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations with warm start for the small toroidal instances disabling the solver's preprocessing, cuts and heuristics.}\label{tab:toroinitsoldisable}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
Toro\_5\_5\_10\_25 & 232.8 & 5 & 1.3 &  & 232.8 & 5 & 0.9 &  & 232.8 & 5 & 0.0 &  & 232.8 & 5 & 0.1 &  & 232.8 & 5 & 1.6 &  \\ 
  Toro\_5\_5\_10\_50 & 357.2 & 5 & 1.2 &  & 357.2 & 5 & 0.9 &  & 357.2 & 5 & \textbf{0.0} &  & 357.2 & 5 & \textbf{0.0} &  & 357.2 & 5 & 1.5 &  \\ 
  Toro\_5\_5\_10\_75 & 448.6 & 5 & 1.2 &  & 448.6 & 5 & 0.9 &  & 448.6 & 5 & \textbf{0.0} &  & 448.6 & 5 & 0.1 &  & 448.6 & 5 & 1.6 &  \\ \hline
  Toro\_7\_7\_10\_25 & 471.2 & 5 & 7.4 &  & 471.2 & 5 & 1.4 &  & 471.2 & 5 & \textbf{0.6} &  & 471.2 & 5 & 1.3 &  & 471.2 & 5 & 1.9 &  \\ 
  Toro\_7\_7\_10\_50 & 734.6 & 5 & 1.6 &  & 734.6 & 5 & 1.0 &  & 734.6 & 5 & \textbf{0.2} &  & 734.6 & 5 & 0.4 &  & 734.6 & 5 & 1.7 &  \\ 
  Toro\_7\_7\_10\_75 & 912.4 & 5 & 1.5 &  & 912.4 & 5 & 1.0 &  & 912.4 & 5 & \textbf{0.2} &  & 912.4 & 5 & 0.3 &  & 912.4 & 5 & 1.9 &  \\ \hline
  Toro\_9\_9\_10\_25 & 730.0 & 0 &  & 2.3 & 730.0 & 5 & 24.0 &  & 730.0 & 5 & \textbf{18.6} &  & 730.0 & 5 & 32.5 &  & 730.0 & 5 & 26.3 &  \\ 
  Toro\_9\_9\_10\_50 & 1130.4 & 5 & 120.3 &  & 1130.4 & 5 & 1.9 &  & 1130.4 & 5 & \textbf{1.8} &  & 1130.4 & 5 & 5.2 &  & 1130.4 & 5 & 4.1 &  \\ 
  Toro\_9\_9\_10\_75 & 1478.6 & 5 & 35.5 &  & 1478.6 & 5 & 1.6 &  & 1478.6 & 5 & \textbf{1.5} &  & 1478.6 & 5 & 3.2 &  & 1478.6 & 5 & 6.1 &  \\ \hline
  Average & 721.8 &  & 21.3 & 2.3 & 721.8 &  & 3.7 &  & 721.8 &  & 2.6 &  & 721.8 &  & 4.8 &  & 721.8 &  & 5.2 &  \\ 
  Total &  & 40 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  &  & 45 &  &  \\ 
   \hline
\end{tabular}
\end{table}


\begin{table}[H]
\centering
\scriptsize
\caption{Results comparing the formulations with warm start for the small random instances disabling the solver's preprocessing, cuts and heuristics.}\label{tab:randinitsoldisable}
\begin{tabular}{l|rrrr|rrrr|rrrr|rrrr|rrrr}
  \hline
  & \multicolumn{4}{c|}{CYC} & \multicolumn{4}{c|}{TCYC} & \multicolumn{4}{c|}{FLOW} & \multicolumn{4}{c|}{MTZ} & \multicolumn{4}{c}{DCUT} \\ 
Instance & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap & avg & opt & time & gap \\
group &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) &  &  & (s) & (\%) \\
  \hline
R\_25\_33\_10\_25 & 317.2 & 5 & 1.4 &  & 317.2 & 5 & 1.1 &  & 317.2 & 5 & \textbf{0.0} &  & 317.2 & 5 & 0.1 &  & 317.2 & 5 & 1.7 &  \\ 
  R\_25\_33\_10\_50 & 525.8 & 5 & 1.4 &  & 525.8 & 5 & 1.1 &  & 525.8 & 5 & \textbf{0.0} &  & 525.8 & 5 & \textbf{0.0} &  & 525.8 & 5 & 1.7 &  \\ 
  R\_25\_33\_10\_75 & 702.8 & 5 & 1.4 &  & 702.8 & 5 & 1.1 &  & 702.8 & 5 & \textbf{0.0} &  & 702.8 & 5 & \textbf{0.0} &  & 702.8 & 5 & 1.4 &  \\ \hline
  R\_25\_69\_10\_25 & 243.0 & 5 & 1.5 &  & 243.0 & 5 & 1.1 &  & 243.0 & 5 & \textbf{0.1} &  & 243.0 & 5 & \textbf{0.1} &  & 243.0 & 5 & 1.8 &  \\ 
  R\_25\_69\_10\_50 & 389.8 & 5 & 1.5 &  & 389.8 & 5 & 1.1 &  & 389.8 & 5 & \textbf{0.1} &  & 389.8 & 5 & \textbf{0.1} &  & 389.8 & 5 & 1.8 &  \\ 
  R\_25\_69\_10\_75 & 597.2 & 5 & 1.4 &  & 597.2 & 5 & 1.1 &  & 597.2 & 5 & \textbf{0.1} &  & 597.2 & 5 & \textbf{0.1} &  & 597.2 & 5 & 1.8 &  \\ \hline
  R\_25\_204\_10\_25 & 106.8 & 5 & 2.0 &  & 106.8 & 5 & 1.3 &  & 106.8 & 5 & 1.4 &  & 106.8 & 5 & \textbf{0.7} &  & 106.8 & 5 & 2.1 &  \\ 
  R\_25\_204\_10\_50 & 193.0 & 5 & 1.8 &  & 193.0 & 5 & 1.3 &  & 193.0 & 5 & 1.2 &  & 193.0 & 5 & \textbf{0.6} &  & 193.0 & 5 & 2.0 &  \\ 
  R\_25\_204\_10\_75 & 312.2 & 5 & 1.8 &  & 312.2 & 5 & 1.3 &  & 312.2 & 5 & 1.2 &  & 312.2 & 5 & \textbf{0.5} &  & 312.2 & 5 & 2.0 &  \\ \hline
  R\_50\_85\_10\_25 & 583.2 & 5 & 2.5 &  & 583.2 & 5 & 1.2 &  & 583.2 & 5 & \textbf{0.1} &  & 583.2 & 5 & 0.4 &  & 583.2 & 5 & 1.8 &  \\ 
  R\_50\_85\_10\_50 & 957.2 & 5 & 1.9 &  & 957.2 & 5 & 1.2 &  & 957.2 & 5 & \textbf{0.1} &  & 957.2 & 5 & 0.4 &  & 957.2 & 5 & 1.9 &  \\ 
  R\_50\_85\_10\_75 & 1229.8 & 5 & 1.7 &  & 1229.8 & 5 & 1.1 &  & 1229.8 & 5 & \textbf{0.1} &  & 1229.8 & 5 & 0.3 &  & 1229.8 & 5 & 1.8 &  \\ \hline
  R\_50\_232\_10\_25 & 355.2 & 5 & 325.4 &  & 355.2 & 5 & \textbf{6.8} &  & 355.2 & 5 & 34.1 &  & 355.2 & 5 & 11.5 &  & 355.2 & 5 & 10.6 &  \\ 
  R\_50\_232\_10\_50 & 657.2 & 5 & 123.3 &  & 657.2 & 5 & \textbf{5.1} &  & 657.2 & 5 & 16.8 &  & 657.2 & 5 & 7.0 &  & 657.2 & 5 & 6.5 &  \\ 
  R\_50\_232\_10\_75 & 889.6 & 5 & 91.9 &  & 889.6 & 5 & \textbf{4.2} &  & 889.6 & 5 & 15.4 &  & 889.6 & 5 & 5.6 &  & 889.6 & 5 & 7.7 &  \\ \hline
  R\_50\_784\_10\_25 & 146.4 & 5 & 449.9 &  & 146.4 & 5 & \textbf{15.7} &  & 146.4 & 5 & 220.5 &  & 146.4 & 5 & 68.0 &  & 146.4 & 5 & 32.9 &  \\ 
  R\_50\_784\_10\_50 & 278.2 & 5 & 294.3 &  & 278.2 & 5 & \textbf{14.7} &  & 278.2 & 5 & 193.3 &  & 278.2 & 5 & 61.4 &  & 278.2 & 5 & 31.2 &  \\ 
  R\_50\_784\_10\_75 & 415.6 & 5 & 243.9 &  & 415.6 & 5 & \textbf{13.5} &  & 415.6 & 5 & 168.1 &  & 415.6 & 5 & 53.8 &  & 415.6 & 5 & 30.4 &  \\ \hline
  R\_75\_157\_10\_25 & 792.0 & 4 & 730.2 & 2.4 & 792.0 & 5 & 5.5 &  & 792.0 & 5 & \textbf{1.3} &  & 792.0 & 5 & 5.1 &  & 792.0 & 5 & 2.7 &  \\ 
  R\_75\_157\_10\_50 & 1250.6 & 5 & 783.1 &  & 1250.6 & 5 & 3.7 &  & 1250.6 & 5 & \textbf{2.1} &  & 1250.6 & 5 & 3.6 &  & 1250.6 & 5 & 2.7 &  \\ 
  R\_75\_157\_10\_75 & 1870.6 & 5 & 189.5 &  & 1870.6 & 5 & 2.0 &  & 1870.6 & 5 & \textbf{1.5} &  & 1870.6 & 5 & 2.7 &  & 1870.6 & 5 & 5.8 &  \\ \hline
  R\_75\_490\_10\_25 & 461.8 & 0 &  & 20.1 & 461.8 & 5 & \textbf{704.1} &  & 461.8 & 4 & 2046.1 & 8.3 & 461.8 & 5 & 794.4 &  & 461.8 & 5 & 719.9 &  \\ 
  R\_75\_490\_10\_50 & 797.4 & 0 &  & 21.9 & 797.4 & 5 & 805.0 &  & 797.4 & 4 & 2391.7 & 3.3 & 797.4 & 5 & 784.5 &  & 797.4 & 5 & \textbf{624.1} &  \\ 
  R\_75\_490\_10\_75 & 1233.4 & 0 &  & 17.2 & 1233.4 & 5 & \textbf{287.3} &  & 1233.4 & 5 & 1274.5 &  & 1233.4 & 5 & 367.1 &  & 1233.4 & 5 & 387.6 &  \\ \hline
  R\_75\_1739\_10\_25 & 158.4 & 0 &  & 55.9 & 158.4 & 5 & \textbf{162.8} &  & 158.4 & 3 & 2724.3 & 21.8 & 158.4 & 5 & 901.4 &  & 158.4 & 5 & 418.2 &  \\ 
  R\_75\_1739\_10\_50 & 300.4 & 0 &  & 51.3 & 300.4 & 5 & \textbf{124.4} &  & 300.4 & 5 & 2304.4 &  & 300.4 & 5 & 693.4 &  & 300.4 & 5 & 352.0 &  \\ 
  R\_75\_1739\_10\_75 & 458.2 & 0 &  & 49.2 & 458.2 & 5 & \textbf{119.4} &  & 458.2 & 5 & 2087.2 &  & 458.2 & 5 & 555.5 &  & 458.2 & 5 & 297.3 &  \\ \hline
  Average & 600.9 &  & 154.8 & 31.1 & 600.9 &  & 84.7 &  & 600.9 &  & 499.5 & 11.1 & 600.9 &  & 159.9 &  & 600.9 &  & 109.3 &  \\ 
  Total &  & 104 &  &  &  & 135 &  &  &  & 131 &  &  &  & 135 &  &  &  & 135 &  &  \\ 
   \hline
\end{tabular}
\end{table}

\end{landscape}

The plot in Figure~\ref{fig:percincreasetime_Small_disablesolver}
displays the average increase in time in percent over all individual small instances %\celsoF{Confere?}\rafaelF{Aqui é tempo para todas, resolvidas à otimalidade ou não, no mesmo padrão da outra figura de tempo.} 
in each class for each formulation and using the feasible warm starts generated by the matheuristic MILS$^+$-$mtz$ described in Section 3.6 of~\citeA{MelQueRib21}, when the solver's features are disabled.
%It shows that, overall, \textcolor{blue}{TCYC}\rafaelF{Isso é para deixar azul mesmo?} is the formulation mostly affected by the removal of the solver's features.

\begin{figure}[h!]
\begin{center}
%    \begin{tabular}{cc}
    \includegraphics[width=0.6\textwidth]{percincreasetime_Small_disablesolver.pdf}
%  (a) Aggregated results for small instances  & (b) Aggregated results for small instances\\    running as standalone formulations & with warm starts
%\end{tabular}
\end{center}
\caption{Average increase in time in percent over all individual small instances in each class for each formulation and using the feasible warm starts, when the solver's features are disabled.}\label{fig:percincreasetime_Small_disablesolver}
\end{figure}
\rafaelF{reason to only use flow and mtz without clique inequalities}


